Efficient SimRank Computation via Linearization

SimRank, proposed by Jeh and Widom, provides a good similarity measure that has been successfully used in numerous applications. While there are many algorithms proposed for computing SimRank, their computational costs are very high. In this paper, we propose a new computational technique, "SimRank linearization," for computing SimRank, which converts the SimRank problem to a linear equation problem. By using this technique, we can solve many SimRank problems, such as single-pair compuation, single-source computation, all-pairs computation, top k searching, and similarity join problems, efficiently.

==> icde/abstract.tex <==
\begin{abstract}
Similarity join finds all pairs of objects $(i,j)$
with similarity score $s(i,j)$ greater than some specified threshold $\theta$.
This is a fundamental query problem in the database research community,
and is used in many practical applications,
such as duplicate detection, merge/purge, record linkage, object matching,
and reference conciliation.

In this paper,
we propose a scalable algorithm for the similarity join problem with the SimRank similarity measure.
The algorithm consists of two phases: filter and verification.
The filter phase enumerates similar pair candidates,
and the similarity of each candidate is then assessed in the verification phase.

The scalability of the proposed algorithm is experimentally verified for large real networks.
The complexity depends only on the number of similar pairs, but does not depend on all pairs $O(n^2)$.
The proposed algorithm scales up to the network of 5M vertices and 70M edges.
By comparing the state-of-the-art algorithms, it is about 10 times faster
and it requires about 10 times smaller memory.
%The proposed algorithm is 10 to 20 times faster, and requires only 10 to 20 times smaller memory that of the state-of-the-arts algorithms, and scales up to the network of about 5M vertices and 70M edges.


%The filter phase is the important phase of the proposed algorithm.
%Unlike similarity join with Jaccard similarity,
%SimRank utilizes the multi hop neighborhood information.
%Therefore, enumerating the candidates of similar pairs is a nontrivial task.
%For this purpose, we first apply the linearization of the SimRank.
%We then adopt the Gauss-Southwell algorithm,
%a classical method for solving linear equations,
%to compute the relevant scores of SimRank.
%%
%The bottleneck in this method is the memory allocation.
%To upscale the method, we introduce a novel stochastic memory-reducing technique,
%which guarantees that
%the result is very likely to approximate the exact result.
%
%After the filter phase,
%the similarity of the candidates is verified by a Monte-Carlo algorithm.
%The number of Monte-Carlo samples is adaptively controlled by
%observing the Hoeffding inequality.
\end{abstract}


==> icde/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we propose a scalable algorithm for the similarity join problem with SimRank.
The proposed algorithm follows the filter-and-verification framework,
and is adopted the following techniques: 1) the linearization of the SimRank, 2) the Gauss-Southwell algorithm, 3) stochastic thresholding, 4) Monte-Carlo simulation in parallel, and 5) adaptively increased Monte-Carlo samples.

We conducted experiments on large real datasets.
The complexity depends only on the number of similar pairs, but does not depend on all pairs $O(n^2)$;
hence the proposed algorithm scales up to the network of 5M vertices and 70M edges.
By comparing the state-of-the-art algorithms, 
it is about 10 times faster, and it requires about 10 times smaller memory.

%The proposed algorithm consists of two phases: filter phase and verification phase.
%We enumerate the candidates of similar pairs in filter phase and
%examine that each candidates is really similar or dissimilar in verification phase.
%For the filter phase, we combine three techniques: 1) the linearization of SimRank, 2) the Gauss-Southwell algorithm, and 3) stochastic thresholding.
%For the verification phase, we adopt a Monte-Carlo algorithm,
%where the number of Monte-Carlo samples is adaptively controlled.
%
%We conducted numerical experiments to evaluates the proposed algorithm.
%We showed that the algorithm scales up to the network of 1M vertices and 10M edges.


==> icde/experiments3.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we perform numerical experiments to evaluate the proposed algorithm.

\begin{table*}[tb]
\caption{Scalability of the proposed algorithm.}
\label{tbl:scalability}
\centering
\input{icde/tbl_scalability}
\end{table*}

We used the datasets shown in Table~\ref{tbl:scalability}.
These are obtained by Stanford Large Network Dataset Collection\footnote{\textit{https://snap.stanford.edu/data/}}.
%\input{dataset_table}

All experiments were conducted on an Intel Xeon E5-2690
2.90GHz CPU (32 cores) with 256GB memory running Ubuntu 12.04.
The proposed algorithm was implemented in C++ and was compiled
using g++v4.6 with the -O3 option.
We have used OpenMP for parallel implementation.


\subsection{Scalability}

We first show that the proposed algorithm is scalable.
For real datasets,
we compute the number of pairs that has the SimRank score greater than $\theta = 0.2$,
where the parameters of the algorithm are set to the following.
\begin{itemize}
  \item For the filter phase, accuracy parameter for the Gauss-Southwell algorithm (Algorithm~\ref{alg:gausssouthwell}) is set to $\gamma = 0$, and the skip parameter $\beta$ for the stochastic thresholding (Algorithm~\ref{alg:thresholding}) is set to $\beta = 100$.
  \item For the verification phase, the tolerance probability $p$ is set to $p = 0.01$ and the maximum number of Monte-Carlo samples is set to $R_{\mathrm{max}} = 1000$.
\end{itemize}
%We computed the number of similar pairs by proposed algorithm for various real datasets;
%the largest instance, as-skitter, has $|V| = 1,696,145$ vertices and $|E| = 11,095,298$ edges.
The result is shown in Table~\ref{tbl:scalability},
which is the main result of this paper.
Here, ``dataset'', ``$|V|$'', and ``$|E|$'' denote the statistics of dataset,
``$|J_L|$'' and ``$|J_H|$'' denote the size of $J_L$ and $J_H$ in \eqref{eq:JLJH},
``estimate'' denotes the number of similar pairs estimated by the algorithm,
``filter'' and ``verification'' denote the real time needed to compute filter and verification step,
and ``memory'' denotes the allocated memory during the algorithm.

This shows the proposed algorithm is very scalable.
In fact, it can find the SimRank join for the networks of
5M vertices and 68M edges (``soc-LiveJournal'') in a 1000 seconds with 23 GB memory.

Let us look into the details.
The computational time and the allocated memory depend on the number of the similar pairs,
and even if the size of two networks are similar, the number of similar pairs in these networks can be very different.
%Even for the similar size networks, the number of similar pairs can be very different.
For example, the largest instance examined in the experiment is
``soc-LiveJournal'', which has 5M vertices and 68M edges.
However, since it has a small number of similar pairs,
we can compute the SimRank join.
On the other hand, ``web-BerkStan'' dataset, which has only 0.6M vertices and 7M edges,
we cannot compute the SimRank join because it has too many similar pairs.



\subsection{Accuracy}

Next, we verify the accuracy (and the correctness) of the proposed algorithm.
We first compute the exact SimRank scores $S^*$ by using the original SimRank algorithm (Algorithm~\ref{alg:originalsimrank}).
Then, we compare the exact scores with the solution $S$ obtained by the proposed algorithm.
Here, the accuracy of the solution is measured by the precision, the recall, and the F-score~\cite{baeza1999modern}, defined by
\begin{align*}
  \text{precision} = \frac{|S \cap S^*|}{|S|}, \
  \text{recall}    = \frac{|S \cap S^*|}{|S^*|}, \
  \text{F}         = \frac{2 |S \cap S^*|}{|S|+|S^*|}.
\end{align*}
We use the same parameters as the previous subsection.
Since all-pairs SimRank computation is expensive,
we used relatively small datasets for this experiment.

The result is shown in Table~\ref{tbl:accuracy}.
This shows the proposed algorithm is very accurate;
the obtained solutions have about $\text{precision} \approx 97\%$, $\text{recall} \approx 92\%$, and $\text{F-score} \approx 95\%$.
Since the precision is higher than the recall,
the algorithm produces really similar pairs.
%observe that the pairs obtained ths algorithm
%is
%proposed algorithm is conservative, i.e.,
%pairs obtained by the proposed algorithm is really similar.

%% trick !!
%\begin{table}[tb]
%\caption{Accuracy of the proposed algorithm.}
%\label{tbl:accuracy}
%\centering
%\input{tbl_accuracy}
%\end{table}


\subsection{Comparison with the state-of-the-arts algorithms}


We then compare the proposed algorithm with some state-of-the-arts algorithms.
For the proposed algorithm, we used the same parameters described in the previous section.
For the state-of-the-arts algorithms, we implemented the following two algorithms%
\footnote{
We have also implemented the Sun et al.~\cite{sun2011link}'s LS-join algorithm;
however, it did not return a solution even for the smallest instance (ca-GrQc).
The reason is that their algorithm is optimized to find the top-$k$ (with $k \le 100$) similar pairs between given two small sets.}:
\begin{enumerate}
  \item
    Yu et al.~\cite{yu2010taming}'s all-pairs SimRank algorithm.
    This algorithm computes all-pairs SimRank in $O(n m)$ time and $O(n^2)$ space.
    As discussed in \cite{yu2010taming}, we combine thresholding heuristics that discard small values (say $0.01$) in the SimRank matrix for each iteration.
    For the SimRank join, we first apply this algorithm and then output the similar pairs.

  \item
    Fogaras and Racz~\cite{fogaras2005scaling}'s random-walk based single-source SimRank algorithm.
    This algorithm computes single-source SimRank in $O(m)$ time and $O(n R)$ space, where $R$ is the number of Monte-Carlo samples.
    We set the number of Monte-Carlo samples $R = 1000$.
    For the SimRank join, we perform single-source SimRank computations for all seed vertices in parallel, and then output the similar pairs.
\end{enumerate}
We chose the parameters of these algorithms to hold similar accuracy (i.e., $\text{F-score} \approx 95\%$).
%
We used 7 datasets (3 small and 4 large datasets).
For small datasets, we also compute the exact SimRank scores and evaluate the accuracy.
For large datasets, we only compare the scalability.

The result is shown in Table~\ref{tbl:comparison};
each cell denotes the computational time, the allocated memory, and the F-score (for small datasets) or the number of similar pairs (for large datasets), respectively.
``---'' denotes the algorithm did not return a solution within 3 hour and 256 GB memory.

The results of small instances show that the proposed algorithm performs
the same level of accuracy to the existing algorithms with requiring much smaller memory and comparable time.
For large instances, the proposed algorithm outperforms the existing algorithms both in time and space,
because the complexity of the proposed algorithm depends on the number of similar pairs whereas the complexity of existing algorithms depends on the number of pairs, $O(n^2)$.
%For large instances, the proposed algorithm find a solution
%whereas the existing algorithms do not.
This shows the proposed algorithm is very scalable than the existing algorithms.

More precisely, the algorithm is efficient when
the number of similar pairs is relatively small.
For example, in email-Enron and web-Google datasets, which have many similar pairs,
the performance of the proposed algorithm close to
the existing algorithms.
On the other hand, in p2p-Gnutella31 and cit-patent dataset,
it clearly outperforms the existing algorithms.

%%% trick
\begin{table}[tb]
\caption{Accuracy of the proposed algorithm.}
\label{tbl:accuracy}
\centering
\input{icde/tbl_accuracy}
\end{table}


\begin{table}[tb]
\caption{Comparison of algorithms.}
\label{tbl:comparison}
\centering
\input{icde/tbl_comparison}
\end{table}


\subsection{Experimental analysis of our algorithm}

In the previous subsections,
we observed that the proposed algorithm is scalable and accurate.
Moreover, it outperforms the existing algorithms.
In this subsection,
we experimentally evaluate the behavior of the algorithm.

We first evaluate the dependence with the accuracy parameter $\gamma$
used in the Gauss-Southwell algorithm.
We vary $\gamma$ and compute the lower set $J_L$ and the upper set $J_H$.
The result is shown in Table~\ref{tbl:gamma};
each cell denotes the computational time, the allocated memory, and the size of $J_L$ and $J_H$, respectively.

This shows, to obtain an accurate upper and lower sets,
we need to set $\gamma \ge 0.9$.
However, it requires $5$ times longer computational time
and $10$ times larger memory.
Since the verification phase can be performed in parallel,
to scale up for large instances,
it would be nice to set a small $\gamma$ (e.g., $\gamma = 0$).


\begin{table}[tb]
\caption{Dependency of accuracy parameter $\gamma$.}
\label{tbl:gamma}
\centering
\input{icde/tbl_gamma}
\end{table}

Next, we evaluate the dependence with the probability parameter $\beta$
in the stochastic thresholding.
We vary the parameter $\beta$ and evaluate the used memory.
The result is shown in Table~\ref{tbl:memory_reducing}.
The column for $\beta = \infty$ shows the result without this technique.
Thus we compare other columns with this column.
The result shows that the effect of memory-reducing technique
greatly depends on the network structure.
However, for an effective case, it reduces memory about $1/2$.
By setting $\beta = 100$, we can obtain almost the same result as
the result without the technique.

\begin{table}[tb]
\caption{Dependency of the parameter $\beta$ for the stochastic thresholding.}
\label{tbl:memory_reducing}
\centering
\input{icde/tbl_memory_reducing}
\end{table}

Finally, we evaluate the effectiveness of the adaptive Monte-Carlo samples technique in the verification phase.
We plot the histogram of the number of required samples in Figure~\ref{fig:required_samples}. Here, the bar at 1,000 denotes the candidates that cannot be decided in 1,000 samples.

The result shows that most of small candidates are decided in 200 samples,
and $1/3$ of samples cannot decided in 1,000 samples.
Therefore, this implies the technique of
adaptive Monte-Carlo samples reduces
the computational cost in factor about $1/3$.

\begin{figure}[tb]
\centering
\input{icde/fig_required_samples}
\caption{Histogram of the number of required samples.}
\label{fig:required_samples}
\end{figure}


%\section{Applications}
%
%In this section, we demonstrate the proposed algorithm in some applications.
%
%
%\subsection{Near duplication detection}
%
%As mentioned in Introduction, the fundamental application of the similarity join query is the near-duplicate detection problem.
%Here, we demonstrate the proposed algorithm in this application.
%
%We use web-NotreDame dataset, which represents a web-graph in University of Notre Dame.
%The network consists of $281903$ vertices and $2312497$ edges;
%see \cite{albert1999internet} for details of this dataset.
%%
%We construct a network as follows:
%We randomly select 28190 ($10\%$) vertices, and clone these vertices with these links.
%The obtained network $\tilde G$ consists of 310093 (=281903+28190) vertices.
%The task is to detect these cloned vertices from the network.
%
%We compute SimRank join for the reversed graph $\tilde G^\top$ with various threshold $\theta$.
%The result is shown in Table~\ref{tbl:duplicate}.
%We obtained $XXX$ similar pairs candidate, and it contains all cloned vertices.
%
%\begin{table}[tb]
%\caption{Near duplicate detection.}
%\label{tbl:duplicate}
%\centering
%\input{tbl_duplicate}
%\end{table}
%


\subsection{Number of similar pairs}

Cai et al.~\cite{cai2009efficient} claimed that
the SimRank scores of a network follows power-law distributions.
However, they only verified this claim in small networks (at most 10K vertices).

We here verify this conjecture in larger networks.
We first enumerate the pairs with SimRank greater than $\theta = 0.001$,
and then compute the SimRank score by the Monte-Carlo algorithm.
%We compute the number of similar pairs
%by varying the similarity threshold $\theta$.
The result is shown in Figure~\ref{fig:number_of_similar_pairs}.
This shows, for each experimented dataset,
the number of similar pairs follows power-law distributions in this range;
however, these exponent (i.e., the slope of each curve) are different.


%\begin{table}[tb]
%\caption{Number of similar pairs.}
%\label{tbl:number_of_similar_pairs}
%\centering
%\input{tbl_number_of_similar_pairs}
%\end{table}

\begin{figure}[tb]
\input{icde/fig_similarpairs}
\caption{The number of similar pairs.}
\label{fig:number_of_similar_pairs}
\end{figure}


%% vim:foldmethod=marker


==> icde/filter.tex <==
\section{Filter phase}
\label{sec:filter_top}

\begin{algorithm}[tb]
\caption{SimRank join algorithm.}
\label{alg:simrankjoin}
\begin{algorithmic}[1]
\Procedure{SimRankJoin}{$\theta$}
\State{Compute two sets $J_L$ and $J_H$.}
\State{Output all $(i,j) \in J_L$.}
\For{$(i,j) \in J_H \setminus J_L$}
\If{$i$ and $j$ are really similar}
\State{Output $(i,j)$.}
\EndIf
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

In this section, we discuss the details of the filter phase
for enumerating similar-pair candidates.
We will discuss the details of the verification phase in the next section. 
Let us give overview of the filter phase. 

Let $J(\theta) = \{ (i,j) : s(i,j) \ge \theta \}$ be the set of similar pairs.
The filter phase produces two subsets $J_L(\theta,\gamma)$ and $J_H(\theta,\gamma)$ such that
\begin{align}
\label{eq:JLJH}
  J_L(\theta,\gamma) \subseteq J(\theta) \subseteq J_H(\theta,\gamma),
\end{align}
where $\gamma \in [0,1]$ is an accuracy parameter.
Here,
$J_L(\theta,\gamma)$ is monotone increasing in $\gamma$,
$J_H(\theta, \gamma)$ is monotone decreasing in $\gamma$,
and $J_L(\theta,1) = J(\theta) = J_H(\theta,1)$.
%
%Since we cannot determine a pair $(i,j) \in J_H(\theta,\gamma) \setminus J_L(\theta,\gamma)$ is really similar or not,
%we check all such candidates in the verification phase. (see Algorithm~\ref{alg:simrankjoin}).
%
Note that, our filter phase gives 100\%-precision solution $J_L(\theta,\gamma)$ and 100\%-recall solution $J_H(\theta,\gamma)$.
These two sets might be useful in some applications.

Let us consider how to implement the filter phase.
The basic idea is that ``compute only relevant entries of SimRank.''
In order to achieve this idea, we combine the two techniques,
the \emph{linearization of the SimRank}~\cite{kusumoto2014scalable,maehara2014efficient},
and
the \emph{Gauss-Southwell algorithm}~\cite{southwell1940relaxation,southwell1946relaxation} for solving a linear equation.
%
The linearization of the SimRank
is a technique to convert a SimRank problem to a linear equation problem.
By using this technique,
the problem of computing large entries of SimRank
is transformed to the problem of computing large entries
of a solution of a linear equation.
To solve this linear algebraic problem,
we can use the Guass-Southwell algorithm.
By error analysis of the Guass-Southwell algorithm (given later in this paper),
our filter algorithm obtains the lower and the upper bound of the SimRank of each pair $(i,j)$.
Using these bounds, the desired sets $J_L(\theta,\gamma)$ and $J_H(\theta,\gamma)$ are obtained, where $\gamma$ is an accuracy parameter used in the Guass-Southwell algorithm.


The above procedure is already much efficient;
however, we want to scale up the algorithm for large networks.
The bottleneck of the above procedure is the memory allocation.
We resolve this issue by introducing the \emph{stochastic thresholding} technique.

This is the overview of the proposed filter phase.
In the following subsections, we give details of the filter phase.



\subsection{Linearized SimRank}
\label{sec:linearizedsimrank}

Here, we describe the linearization of the SimRank proposed in~\cite{maehara2014efficient,kusumoto2014scalable}.
To simplify the notation,
we first introduce matrix representation of SimRank.
Let $S := (s(i,j))_{ij}$ be a matrix of the SimRank entries,
and let $P$ be the transition matrix of the transposed graph of $G = (V, E)$,
defined by
\begin{align}
  P_{ij} := \begin{cases} 1 / I(j), & (i,j) \in E, \\ 0, & \textrm{otherwise}. \end{cases}
\end{align}
Then the definition of the SimRank \eqref{eq:simrankoriginal} is equivalent to
the following matrix equation
\begin{align} \label{eq:nonlinearsimrank}
  S := (c P^\top S P) \lor I,
\end{align}
where $\lor$ denotes the element-wise maximum, i.e., $(A \lor B)_{ij} = \max \{ A_{ij}, B_{ij} \}$,
and $I$ denotes the identity matrix.

SimRank is rendered difficult to solve because of
the \emph{nonlinearity} of \eqref{eq:nonlinearsimrank} introduced by the element-wise maximum.
Thus we reformulate this nonlinear equation as a linear equation.
Let us compare the left with the right hand sides of \eqref{eq:nonlinearsimrank}.
Since the maximum with $I$ only affects the diagonals,
the off-diagonal entries of $S$ and $c P^\top S P$ are the same.
Therefore there exists a diagonal matrix $D$ such that
\begin{align} \label{eq:linearizedsimrank}
  S = c P^\top S P + D.
\end{align}
This matrix $D$ is called the \emph{diagonal correction matrix}.%
\footnote{Some existing studies have been used $D = (1 -c) I$; however, this gives a wrong SimRank score. See~\cite{maehara2014efficient}.}
Having obtained $D$,
we can analyze SimRank via the linear equation~\eqref{eq:linearizedsimrank}.
On the basis of \eqref{eq:linearizedsimrank}, we can develop efficient algorithms for computing
single pair and single source queries in SimRank.

The remaining problem is how to estimate the diagonal correction matrix $D$.
To avoid confusion,
we denote a matrix that satisfies the relation \eqref{eq:linearizedsimrank} for a given matrix $D$ by $S(D)$;
the task is to find a matrix $D$ such that $S(D)$ is equal to the SimRank matrix $S$.
$D$ is uniquely determined by the condition:
\begin{align}
  \label{eq:condition}
  S(D)_{kk} = 1 \textrm{ for all } k \in V.
\end{align}
This condition is a linear equation in $D$ because the matrix $S(D)$ satisfying \eqref{eq:linearizedsimrank} is linear in $D$.
Therefore $D$ can be computed by an algorithm in numerical linear algebra.
We here apply the Gauss-Seidel algorithm~\cite{golub2012matrix} with Monte-Carlo simulations.
The algorithm initially sets $D = I$,
then iteratively updates $D$ subject to \eqref{eq:condition}.
More precisely,
for each $k \in V$,
$D_{kk}$ is updated as $D_{kk} + \delta$ such that $S(D)_{kk} = 1$.
Here, $\delta$ is determined by
\begin{align}
  S(D + \delta e_i e_i^\top)_{kk} = 1,
\end{align}
i.e.,
\begin{align}
  \label{eq:delta}
  \delta = \frac{1 - S(D)_{kk}}{S(e_k e_k^\top)_{kk}}.
\end{align}
To evaluate the right hand side of \eqref{eq:delta},
we require to compute $S(D)_{kk}$ and $S(e_k e_k^\top)_{kk}$.
From \eqref{eq:linearizedsimrank}, we have
\begin{align}
  \label{eq:expansion}
  S(D)_{kk} = \sum_{k=0}^\infty c^k (P^k e_i)^\top D (P^k e_i),
\end{align}
where the sum is usually truncated about $k \le 10$.
By approximating $P^k e_i$ using Monte-Carlo samples,
we can efficiently update $D_{kk}$.
By repeating this procedure until convergence,
we obtain an algorithm that estimates the correction matrix $D$.
The precise implementations are shown in Algorithms~\ref{alg:Diagonal} and \ref{alg:DiagonalAlphaBeta}.
The convergence proof and error analysis are presented in \cite{maehara2014efficient}.

\begin{algorithm}[tb]
\caption{Diagonal estimation algorithm~\cite{maehara2014efficient}.}
\label{alg:Diagonal}
\begin{algorithmic}[1]
\Procedure{DiagonalEstimation}{}
\State{$D = I$.}
\For{$\ell = 1, \ldots, L$}
\For{$k \in V$}
\State{$\delta \leftarrow$ ComputeDelta($k$)}
\State{$D_{kk} \leftarrow D_{kk} + \delta$}
\EndFor
\EndFor
\State{\Return $D$}
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
\caption{Estimate $S(D)_{kk}$ and $S(e_k e_k^\top)_{kk}$~\cite{maehara2014efficient}.} \label{alg:DiagonalAlphaBeta}
\begin{algorithmic}[1]
\Procedure{ComputeDelta}{$k$}
\State{$\alpha \leftarrow 0$, $\beta \leftarrow 0$,
$k_1 \leftarrow k, k_2 \leftarrow k, \ldots, k_R \leftarrow k$}
\For{$t = 1, 2, \ldots, T$}
\For{$i \in \{ k_1, k_2, \ldots, k_R \}$}
\State{$p_{ki}^{(t)} \leftarrow \# \{ r = 1, \ldots, R : k_r = i \}/R$}
%\State{$p_i^{(t)} \leftarrow \# \{ r : k_r = i, r = 1, \ldots, R \}/R$}
\If{$i = k$}
\State{$\alpha \leftarrow \alpha + c^t p_{ki}^{(t) 2}$}
\EndIf
\State{$\beta \leftarrow \beta + c^t p_{ki}^{(t) 2} D_{i i}$}
\EndFor
\For{$r = 1, \ldots, R$}
\State{$k_r \leftarrow I(k_r)$ randomly}
\EndFor
\EndFor
\State{\Return $\delta \approx (1 - \alpha) / \beta$}
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Gauss-Southwell algorithm}
\label{sec:gausssouthwell}

By the linearization of the SimRank, we obtained the linear equation \eqref{eq:linearizedsimrank}.
We want to solve this linear equation in $S$;
however, since it has $O(n^2)$ variables, we must keep track only on large entries of $S$.
For this purpose, we adopt the Gauss-Southwell algorithm~\cite{southwell1940relaxation,southwell1946relaxation},
which is a very classical algorithm for solving a linear equation.
In this subsection, we describe the Gauss-Southwell algorithm for a general linear equation $A x = b$,
and in the next subsection, we apply this method for the linearized SimRank equation \eqref{eq:linearizedsimrank}.

Suppose we desire an approximate solution to the linear system $A x = b$,
where $A$ is an $n \times n$ matrix with unit diagonal entries,
i.e., $A_{ii} = 1$ for all $i = 1, \ldots, n$.
%
Let $\epsilon > 0$ be an accuracy parameter.
The Gauss-Southwell algorithm is an iterative algorithm.
Let $x^{(t)}$ be the $t$-th solution
and $r^{(t)} := b - A x^{(t)}$ be the corresponding residual.
At each step,
the algorithm chooses an index $i$ such that $|r^{(t)}_i| \ge \epsilon$,
and updates the solution as
\begin{align}
  x^{(t+1)} = x^{(t)} + r^{(t)}_i e_i,
\end{align}
where $e_i$ denotes the $i$-th unit vector.
The corresponding residual becomes
\begin{align}
  r^{(t+1)} = b - A x^{(t+1)} = r^{(t)} - r^{(t)}_i A e_i.
\end{align}
Since $A$ has unit diagonals, the $i$-th entry of $r^{(t+1)}$ is zero.
Repeating this process
until $r^{(t)}_i < \epsilon$ for all $i = 1, \ldots, n$,
we obtain a solution $x$ such that $\| b - A x \|_\infty < \epsilon$.
This algorithm is called the \emph{Gauss-Southwell} algorithm.

Note that this algorithm is recently rediscovered
and applied to the personalized PageRank computation.
See Section~\ref{sec:relatedwork} for related work.


\subsection{Filter phase}
\label{sec:filter}

We now propose our filtering algorithm.
First, we compute the diagonal correction matrix $D$ by Algorithm~\ref{alg:Diagonal},
reducing the SimRank computation problem to the linear equation~\eqref{eq:linearizedsimrank}.
The Gauss-Southwell algorithm is then applied to the equation.

The $t$-th solution $S^{(t)}$ and the corresponding residual $R^{(t)}$ are maintained such that
\begin{align}
  D - (S^{(t)} - c P^\top S^{(t)} P) = R^{(t)}.
\end{align}
Initial conditions are $S^{(0)} = O$ and $R^{(0)} = D$.
At each step, the algorithm finds an entry $(i,j)$ such that $|R^{(t)}_{ij}| \ge \epsilon$,
and then updates the current solution as
\begin{align}
  S^{(t+1)} = S^{(t)} + R^{(t)}_{ij} e_i e_j^\top.
\end{align}
The corresponding residual becomes
\begin{align}
  \label{eq:filteriter}
  R^{(t+1)} = R^{(t)} - R^{(t)}_{ij} e_i e_j^\top + c R^{(t)}_{ij} (P^\top e_i) (P^\top e_j)^\top.
\end{align}
Since we have assumed that $G$ is simple, the $i$-th entry of $P^\top e_i$ is zero,
the $(i,j)$-th entry of $R^{(t+1)}$ is also zero.
The algorithm repeats this process until
$|R^{(t)}_{ij}| < \epsilon$ for all $i,j \in V$.
The procedure is outlined in Algorithm~\ref{alg:gausssouthwell}.

\begin{algorithm}[tb]
\caption{Gauss-Southwell algorithm used in Algorithm~\ref{alg:filter}.}
\label{alg:gausssouthwell}
\begin{algorithmic}[1]
\Procedure{GaussSouthwell}{$\epsilon$}
  \State{$S^{(0)} = O, \, R^{(0)} = D, \, t = 0$}
  \While{there is $(i,j)$ such that $|R^{(t)}_{ij}| > \epsilon$}
  \State{$S^{(t+1)} = S^{(t)} + R^{(t)}_{ij} e_i e_j^\top$}
  \State{$R^{(t+1)} = R^{(t)} - R^{(t)}_{ij} e_i e_j^\top + c R^{(t)}_{ij} (P^\top e_i) (P^\top e_j)^\top$}
  \State{$t \leftarrow t + 1$}
  \EndWhile
  \State{Return $S^{(t)}$ as an approximate SimRank.}
\EndProcedure
\end{algorithmic}
\end{algorithm}

We first show the finite convergence of the algorithm, whose proof will be given in Appendix.
\begin{proposition}
\label{prop:terminate}
Algorithm~\ref{alg:gausssouthwell} terminates at most $t = \Sigma / \epsilon$ steps, where $\Sigma = \sum_{ij} S_{ij}$ is the sum of all SimRank scores.
\end{proposition}
Since the $(i,j)$ step is performed in $O(|I(i)||I(j)|)$ time
with $O(|I(i)||I(j)|)$ memory allocation,
the overall time and space complexity is $O(I_{\mathrm{max}}^2 \Sigma/\epsilon)$,
where $I_{\mathrm{max}}$ is the maximum in-degree of $G$.


We now show that Algorithm 6 guarantees an approximate solution (whose proof will be given in Appendix).
\begin{proposition}
\label{prop:errorestimate}
Let $\gamma \in [0,1)$ be an accuracy parameter and
$\tilde S$ be the approximate SimRank obtained by
Algorithm~\ref{alg:gausssouthwell} with $\epsilon = (1 - c) (1 - \gamma) \theta$.
Then we have
\begin{align}
  \label{eq:errorestimate}
  0 \le S_{ij} - \tilde S_{ij} \le (1 - \gamma) \theta
\end{align}
for all $i, j \in V$.
\end{proposition}
The left inequality
states if $\tilde S_{ij} \ge \theta$, $S_{ij} \ge \theta$.
Similarly, the right inequality states that
if $S_{ij} \ge \theta$, $\tilde S_{ij} \ge \gamma \theta$.
Thus, letting
\begin{align}
  J_L(\theta,\gamma) &:= \{ (i,j) : \tilde S_{ij} \ge \theta \}, \\
  J_H(\theta,\gamma) &:= \{ (i,j) : \tilde S_{ij} \ge \gamma \theta \},
\end{align}
we obtain \eqref{eq:JLJH}.

$J_L$ and $J_H$ can be accurately estimated by letting $\gamma \to 1$.
However, since the complexity is proportional to $O(1/\epsilon) = O(1/(1 - \gamma))$, a large $\gamma$ is precluded.
Therefore, in practice, we set to some small value (e.g., $\gamma = 0$)
and
verify whether the pairs $(i,j) \in J_H(\theta,\gamma) \setminus J_L(\theta,\gamma)$ are actually similar by an alternative algorithm.

\begin{algorithm}[tb]
\caption{Filter procedure.}
\label{alg:filter}
\begin{algorithmic}[1]
\Procedure{Filter}{$\theta$, $\gamma$}
\State{Compute diagonal correction matrix $D$.}
\State{Compute approximate solution $\tilde S$ of linear equation $S = c P^\top S P + D$ by Gauss-Southwell algorithm with accuracy $\epsilon = (1-c) \gamma \theta$.}
\State{Output $J_L = \{ (i,j) : \tilde S_{ij} \ge \theta \}$ and $J_H = \{ (i,j) : \tilde S_{ij} \ge \gamma \theta \}$.}
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Stochastic thresholding for reducing memory}
\label{sec:thresholding}

We cannot predict the required memory before running the algorithm (which depends on the SimRank distribution);
therefore the memory allocation is a real bottleneck
in the filter procedure (Algorithm~\ref{alg:filter}).
To scale up the procedure, we must reduce the waste of memory.
Here, we develop a technique that reduces the space complexity.

We observe that, in Algorithm~\ref{alg:filter}, some entries $R_{ij}$ are only used to store the values,
and never used in future because they do not exceed $\epsilon$;
therefore we want to reduce storing of these values.
Here, a thresholding technique,
which skips memory allocations for very small values, seems effective.
This kind of heuristics is frequently used in SimRank computations~\cite{cai2009efficient,lizorkin2010accuracy,yu2010taming}.
However, a simple thresholding technique may cause large errors because it ignores the accumulation of small values.

To guarantee the theoretical correctness of this heuristics,
we use the \emph{stochastic thresholding} instead of the deterministic thresholding.
When the algorithm requires to allocate a memory,
it skip the allocation with some probability depending on the value (a small value should be skipped with high probability).
Intuitively, if the value is very small, the allocation may be skipped.
However, if there are many small values, one of them may be allocated,
and hence the error is bounded stochastically. The following proposition shows this fact (whose proof will be given in Appendix).

\begin{proposition}
\label{prop:thresholding}
Let $a_1, a_2, \ldots$ be a nonnegative sequence and let $A = \sum_{i=1}^\infty a_i < \infty$.
Let $\beta > 0$.
Let $\tilde A$ be the sum of these values with the stochastic thresholding where the skip probability is $p(a_i) = \min\{1, \beta a_i\}$.
Then we have
\begin{align}
  \P \{ A - \tilde A \ge \delta \} \le \exp(-\beta \delta).
\end{align}
\end{proposition}

We implement the stochastic thresholding (Algorithm~\ref{alg:thresholding}) in Gauss-Southwell algorithm (Algorithm~\ref{alg:gausssouthwell}).
Then, theoretical guarantee in Proposition~\ref{prop:errorestimate} is modified as follows.
\begin{proposition}
\label{prop:memory}
%Let $S$ be the SimRank matrix and let $\tilde S$ be obtained by Algorithm~\ref{alg:gausssouthwell} with Algorithm~\ref{alg:thresholding}.
%Then, for any $i,j \in V$, we have
%\begin{align}
%  0 \le
%  \P\{ |S_{ij} - \tilde S_{ij}| \ge \delta \} \le \exp(-p \delta).
%\end{align}
%\label{prop:errorestimate}
Let $\gamma \in [0,1)$ be an accuracy parameter, $\beta$ be a skip parameter,
and $\tilde S$ be the approximate SimRank obtained by
Algorithm~\ref{alg:gausssouthwell} using stochastic thresholding with $\epsilon = (1 - c) (1 - \gamma) \theta$.
Then we have $ 0 \le S_{ij} - \tilde S_{ij}$ and
\begin{align}
  \P\{ S_{ij} - \tilde S_{ij} \le (1 - \gamma) \theta + \delta \} \le \exp(-(1-c) \beta \delta)
\end{align}
for all $i, j \in V$.
\end{proposition}
Thus, by letting $\beta \propto 1/\delta$, we can reduce the misclassification probability arbitrary small.
%
We experimentally evaluate the effect of this technique
in Section~\ref{sec:experiments}


\begin{algorithm}[tb]
\caption{Stochastic thresholding for $R_{ij} \leftarrow R_{ij} + a$.}
\label{alg:thresholding}
\begin{algorithmic}[1]
  \Procedure{StochasticThresholding}{$R$,$i$,$j$,$a$;$\beta$}
  \If{$R_{ij}$ is already allocated}
  \State{$R_{ij} \leftarrow R_{ij} + a$.}
  \Else
  \State{draw a random number $r \in [0,1]$.}
  \If{$r > \beta a$}
  \State{skip allocation.}
  \Else
  \State{allocate memory for $R_{ij}$ and store $R_{ij} = a$.}
  \EndIf
  \EndIf
  \EndProcedure
\end{algorithmic}
\end{algorithm}


==> icde/preliminaries.tex <==
\section{SimRank}
\label{sec:preliminaries}

This section reviews the SimRank, introduced by Jeh and Widom~\cite{jeh2002simrank} for searching web-pages.

Let $G = (V, E)$ be a directed graph, where 
$V$ is the set of vertices and $E \subseteq V \times V$ is the set of edges.
Through the paper, we assume that $G$ is simple\footnote{This assumption can be removed; however, to simplify the discussion, we assume this.}, i.e., it has no multiple edges and self-loops.
Let $I(i) = \{ j \in V : (j,i) \in E \} $ be the set of in-links of $i \in V$.
The \emph{SimRank score $s(i,j)$ of a pair of vertices $(i, j) \in V \times V$} is 
recursively defined by
\begin{align} \label{eq:simrankoriginal}
s(i,j):= \begin{cases} 1, & i = j, \\ \displaystyle  \frac{c}{|I(i)| |I(j)|} \sum_{i' \in I(i), j \in I(j)} s(i', j'), & i \neq j, \end{cases}
\end{align}
where $c \in \mathbb{R}$ is a decay factor,
usually set to $c = 0.8$~\cite{jeh2002simrank} or $c = 0.6$~\cite{lizorkin2010accuracy}.
%
Jeh and Widom~\cite{jeh2002simrank} proved that definition \eqref{eq:simrankoriginal} is well-defined (i.e., there exists a unique function $s$ satisfies the relation \eqref{eq:simrankoriginal}),
and that Algorithm~\ref{alg:originalsimrank} converges to the SimRank.
SimRank computation algorithms based on the recursion~\eqref{eq:simrankoriginal} have been extensively reported~\cite{jeh2002simrank,lizorkin2010accuracy,yu2010taming}).

SimRank also has a ``random-walk'' interpretation~\cite{jeh2002simrank}.
Consider two random walkers who start from vertices $i$ and $j$
and randomly follow their in-links.
Then the first meeting time of these walkers is denoted by $\tau(i,j)$,
i.e., the walkers first meet at some vertex in step $\tau(i,j)$.
The SimRank score then satisfies
\begin{align}
  \label{eq:randomwalker}
  s(i,j) = \E[ c^{\tau(i,j)} ].
\end{align}
Fogaras and R\'acz~\cite{fogaras2005scaling} proposed
a Monte-Carlo algorithm for computing SimRank on the basis of \eqref{eq:randomwalker}.
Their algorithm efficiently maintains numerous random walks.
An iterative non Monte-Carlo algorithm based on \eqref{eq:randomwalker}
is developed by Li et al.~\cite{li2010fast}. 


\begin{algorithm}[tb]
\caption{Original SimRank algorithm~\cite{jeh2002simrank}.}
\label{alg:originalsimrank}
\begin{algorithmic}[1]
\Procedure{SimRank}{}
\State{$s(i,j) = 0$ for all $i,j$.}
\Repeat
\For{$i \in V, j \in V$}
\If{$i = j$}
\State{$s'(i,j) \leftarrow 1$.}
\Else
\State{$s'(i,j) \leftarrow \displaystyle \frac{c}{|I(i)||I(j)|}\sum_{\substack{i'\in I(i)\\j'\in I(j)}} s(i',j')$.}
\EndIf
\EndFor
\State{$s(i,j) \leftarrow s'(i,j)$ for all $i,j$.}
\Until{convergence}
\State{Return $s$.}
\EndProcedure
\end{algorithmic}
\end{algorithm}

Very recently, the authors proposed the so-called \emph{linearization} technique for the SimRank~\cite{maehara2014efficient,kusumoto2014scalable},
which computes SimRank via a linear equation.
Since this technique is adopted in the filter phase of our proposed algorithm,
it is fully explained in Section~\ref{sec:linearizedsimrank}.


==> icde/rebutal.tex <==
First of all, we thank all the reviewers to read our manuscript
carefully and give insightful comments.
We shall improve the presentation in our revised version.
Now we would like to answer questions raised by the reviewers

 [Assigned_Reviewer_1]
 1)
 > The novelty with respect to a very recent paper on SimRank search algorithms by the same authors [26], which is based on very similar techniques, remains obscure.

 By using techniques in [26], we can compute all-pairs SimRank scores more efficiently
 than any existing method. But the drawback is that we have to enumerate O(n^2) pairs in a
 graph. This is too expensive for the SimRank join problem for large
 networks.

 So the main difficulty of the SimRank join problem is:
   How can we find very similar pairs without enumerating O(n^2) pairs?

 The main contribution of this paper is to overcome this issue by
 adopting Gauss-Southwell method (which is given in III-B). This method is clearly different from [26].
 In fact, to the best of our knowledge, this is the first time to adopt the Gauss-Southwell
 method for the similarity join problem. In addition, the filter phase in IV is totally different (and new).
 So in our view, these two contributions are new and novel (as Reviewers 2&3 agreed).


 2)
 > The SimRank join algorithm [29] is not considered in the experimental evaluation. The discussion of [29] suggests that this algorithm precomputes and stores the result of all-pairs SimRank, which I don't think is true. It seems to be an interesting competitor.
and
W4) of Reviewer_3
 > Reference [29] seems to be described in a wrong way - this paper explicitly states that the join is not materialized; and [29] should be included in the evaluation.

 Actually [29] is the starting point of this work. However, we found one serious issue to adapt the method of [29] for our problem setting. 
 The problem is that [29]'s algorithm consists of offline and online phase (see Fig 4 in
 [29]), and in offline phase, it stores SimRank scores for many pairs of
 vertices. In addition, [29] did not mention how to do that. It seems us that this is possible ONLY IF we can compute SimRank for all-pairs. 

So we asked the authors of [29] about this point. Their answer  is that they actually utilized 
the standard all-pairs algorithm for SimRank. Thus, their algorithm requires at least the same complexity as all-pairs SimRank
computation, which is at least O(n^2). This means that if we do both ``offline phase'' and ``online phase'' of [29], 
the best we can hope is as good as the result of [28] (which is already done in our experiments).  We do not think it fair to do only ``online phase'', 
because the main challenge is to avoid enumerating O(n^2) pairs, as pointed out above. 
To support this fact here, 
please see Table 3 of [29] which only deals with much smaller datasets (than our experiments). 

To confirm our points here, we attach our communications between the authors of [29] and us at the end of this feedback. Please do not 
disclose this part (and this should be confidential). 


 [Assigned_Reviewer_3]
 W2)
 > The paper *must* from the start say that the algorithm computes a approximate answer ...

We will emphasize this point at the beginning of the paper, but we shall also mention that our
methods also give very accurate answers, as qualified by our experiments.

 W3)
 > The memory reduction method is unclear, as you didn't explain how you implement the matrices in first place.

 We have used a hash table to maintain a sparse matrix. This
 approach is called DOK (see:
http://en.wikipedia.org/wiki/Sparse_matrix), which is efficient in our
 case. We will add some comments about this. Thank you very much for pointing out this remark.


 D1)
 > Please explain why your method failed when trying to work on web-BerkStan. Out of memory?
 > Please also explain clearly in V which parts were parallelized.

 Thank you for point out these remarks, and we shall mention some comments in our revised version.
 For web-berkstan, the reason is out of memory.


 Finally, we would like to mention that our paper [26] may be retracted,
 due to some similarity with our paper [24] in the preliminary section (and we carelessly forgot to cite [24]).
 However, there is nothing wrong with the technical contributions in [26] (and people can check the details
 because [26] is still available).
 We will soon provide a journal version of [24] which also contains
 all the contributions of [26], and make it available as a technical report (arxiv) (so that everybody can access).



==> icde/relatedwork.tex <==
\section{Related work}
\label{sec:relatedwork}

%We here discuss the related works of our reseach.

\paragraph{SimRank join}

Until recently, the SimRank join problem is not well studied
because the most of existing SimRank algorithms can only compute the all-pairs SimRank (it requires at least $O(n^2)$ time),
and if we have the all-pairs SimRank, we can obtain the SimRank join in $O(n^2)$ time.
We will review the algorithms for computing SimRank later.

To the best of our knowledge, there are two existing researches that are concerning the SimRank join problem.
Sun et al.\cite{sun2011link} considered the following version of the similarity join problem:
Given two subsets of vertices $P, Q \subseteq V$, find the top-$k$ similar pairs $(i,j) \in P \times Q$ between these subsets.
They solve this problem for a general random walk-based  similarity measure, which includes the personalized PageRank, SimRank, and the discounted hitting time.
Their algorithm adaptively control the depth of random walks.
They computed SimRank join on the network with 37K vertices (``Cora'' dataset).

Zheng et al.~\cite{zheng2013efficient} proposed an efficient index for the SimRank join.
They first compute the all-pairs SimRank, and then store the information to the index efficiently.
Then, the SimRank join query between two set of vertices $P, Q \subseteq V$ can be quickly answered.
They computed SimRank join on the network with 338K vertices and 1040K edges (``Coauthor'' dataset).


\paragraph{SimRank computation}

The efficient computation of the SimRank scores is a long-standing problem,
and many existing algorithms can only compute the all-pairs SimRank
(i.e., these cannot compute the single-pair and the single-source SimRank).

The original algorithm, proposed by Jeh and Widom~\cite{jeh2002simrank},
is based on the recursion~\eqref{eq:simrankoriginal} and takes $O(m^2)$ time and $O(n^2)$ space.
This algorithm is improved by many researchers (e.g., \cite{lizorkin2010accuracy,JCLHD09,YZLZL12,JLZHD10,cai2009efficient,yu2010taming}),
and the state-of-the-arts implementation by Yu et al.~\cite{yu2010taming} requires $O(n m)$ time.
However, it still requires $O(n^2)$ space, therefore it does not scale for large networks.

Fogaras and Racz~\cite{fogaras2005scaling} proposed a Monte-Carlo algorithm based on the representation of the first meeting time~\ref{eq:randomwalker}.
Their algorithm efficiently maintains set of random walks to compute the single-pair and single-source SimRank.


Our recently proposed technique so-called the ``linearized the SimRank''~\cite{maehara2014efficient,kusumoto2014scalable},
reformulates SimRank as a solution of linear equation.
Such a linearization drastically reduces the computational cost of SimRank,
e.g., the single-pair and the single-source SimRank are computed in $O(m)$ time in $O(n+m)$ space.
This technique is heavily used in this paper;
see Section~\ref{sec:linearizedsimrank} for this technique.

%To the best of our knowledge,
%there is no research for the all pairs similarity search problem about SimRank.
%Zheng et al.~\cite{ZZFZC13} studied the related problem, called \emph{similarity join problem}:
%Given two sets of vertices $A, B \subseteq V$ and a threshold $\theta \in \mathbb{R}$;
%Output all pairs $(a,b) \in A \times B$ of $s(a,b) \ge \theta$.
%They proposed an efficient index structure for this problem,
%but it has to compute all-pairs SimRank scores separately.
%Therefore it cannot applied to our problem.



\paragraph{Gauss-Southwell algorithm in data mining}

The Gauss-Southwell algorithm (see Section~\ref{sec:gausssouthwell}) is the key technique of this paper.
This is a classical algorithm for solving a linear equation, extensively studied by Southwell~\cite{southwell1940relaxation,southwell1946relaxation}.
Since the algorithm is intuitive, it is rediscovered several times.

Recently, in the data mining and the network analysis community,
this algorithm is used to compute the personalized PageRank~\cite{jeh2003scaling}
(e.g., McSherry~\cite{mcsherry2005uniform}, Berkhin~\cite{berkhin2006bookmark}, and Andersen et al.~\cite{andersen2008local}).
These algorithms can find the $\epsilon$-approximate personalized PageRank vector in $O(1/\epsilon)$ iterations.
See Bonchi et al.~\cite{bonchi2012fast}, and Kloster and Gleich~\cite{kloster2013fast}
for details of the Gauss-Southwell algorithm.


%Local algorithms are recently studied
%for PageRank~\cite{berkhin2006bookmark,andersen2008local,borgs2012sublinear} and graph clustering~\cite{spielman2013local}.
%These algorithms only access a small part of a network,
%but can compute the solution with desired accuracy.
%The most relevant algorithm for us is the
%the Berkhin's bookmark coloring algorithm~\cite{berkhin2006bookmark}.
%The algorithm selects an entry that has residual greater than $\epsilon$,
%and update the entry.
%This procedure requires $O(d)$ per iteration and $O(1/\epsilon)$ iterations
%for the desired accuracy $\epsilon$.
%It is important that the number of iteration is independent to the size of a network.

%In the view of numerical linear algebra,
%these methods are very close to the Gauss--Southwell method~\cite{southwell1940relaxation,southwell1946relaxation},
%which is a classical method for a linear equation,
%related to the Gauss--Seidel and coordinate descent algorithms~\cite{luo1992convergence}.
%The Gauss--Southwell algorithm selects the greatest residual entry,
%and update the entry.
%So the Birkhin's bookmark coloring algorithm is a modification of
%this method with avoiding heap structure.
%The method is especially efficient when the desired solution vector is sparse,
%and the desired accuracy is $O(10^{-4})$.
%See Subsection~\ref{sec:localalg} for more details.

%
%In brief, our algorithm is the Southwell method for linearized SimRank equation.
%The obtained algorithm necessarily converges,
%and the number is iterations are expected to $O(n/\epsilon)$,
%where $\epsilon$ is the desired accuracy.
%We verify that the algorithm actually finds all similar vertices,
%and the algorithm scale up to a large networks.
%
%One interesting application of our method is the construction of \emph{similarity graph}.
%A similarity graph $H$ is a network whose vertices are the same as $G$, and
%there is an edge $(i,j) \in E(H)$ if $i$ and $j$ are similar (i.e., $s(i,j)$ is large).
%A similarity graph is useful tool in network analysis.
%In practice, similarity graph consists of many small connected components.
%These connected components give the clustering of the original network.
%We demonstrate the analysis using the similarity graph on DBLP (co-author) dataset.


==> icde/tbl_duplicate.tex <==
\begin{tabular}{l|cc} \hline
$\theta$ & \#candidates & \#detected \\ \hline
0.2 & 100 & 0 \% \\
0.1 & 100 & 0 \% \\
0.05 & 100 & 0 \% \\
0.01 & 100 & 0 \% \\
0.005 & 100 & 0 \% \\
0.001 & 100 & 0 \% \\
\hline
\end{tabular}


==> icde/tbl_number_of_similar_pairs.tex <==
\begin{tabular}{l|rr} \hline
  dataset & $\theta$ & \#similar pairs \\ \hline
  as20000102 & $0.200$ & 626409 \\
             & $0.100$ & 1633163 \\
             & $0.050$ & 5371671 \\
             & $0.025$ & 11745950 \\
  \hline
  ca-GrQc    & $0.200$ & 2684 \\
             & $0.100$ & 8803 \\
             & $0.050$ & 20489 \\
             & $0.025$ & 36364 \\
  \hline
  p2p0Gnutella08 & $0.200$ & 8461 \\
                 & $0.100$ & 20398 \\
                 & $0.050$ & 41217 \\
                 & $0.025$ & 73389 \\
\end{tabular}


==> icde/tbl_required_samples.tex <==
\begin{tabular}{l|c} \hline
  dataset & average samples \\ \hline
  ca-GrQc & 30 \\
  ca-GrQc & 30 \\
  ca-GrQc & 30 \\
  ca-GrQc & 30 \\
  ca-GrQc & 30 \\
  ca-GrQc & 30 \\
\hline
\end{tabular}


==> icde/tmp <==

\section{Experiments}
\label{sec:experiments}

In this section, we perform numerical experiments to evaluate the proposed algorithm.
%to show the efficiency and scalability of our proposed algorithm.
%We further verify the conjecture~\cite{cai2009efficient} that SimRank scores follow the power-law distribution.

\begin{table*}[tb]
\caption{Scalability of algorithm.}
\label{tbl:scalability}
\centering
\input{tbl_scalability}
\end{table*}

We used the datasets shown in Table~\ref{tbl:scalability}.
These are obtained by Stanford Large Network Dataset Collection\footnote{\textit{https://snap.stanford.edu/data/}}.
%\input{dataset_table}


All experiments were conducted on an Intel Xeon E5-2690
2.90GHz CPU (32 cores) with 256GB memory running Ubuntu 12.04.
the proposed algorithm was implemented in C++ and was compiled
using g++v4.6 with the -O3 option.
We have used OpenMP for parallel implementation.

\subsection{Scalability}

We first show that the proposed algorithm is scalable.
For real datasets, 
we compute the number of pairs that has the SimRank score greater that $\theta = 0.2$,
where the parameters of the algorithm are set to the following.
\begin{itemize}
  \item for filter phase, accuracy parameter for the Gauss-Southwell algorithm (Algorithm~\ref{alg:gausssouthwell} is set to $\gamma = 0$, and the probability parameter $\beta$ for the stochastic thresholding (Algorithm~\ref{alg:thresholding}) is set to $\beta = 100$.
  \item for verification phase, the tolerance probability $p$ is set to $p = 0.01$ and the maximum number of Monte-Carlo samples is set to $R_{\mathrm{max}} = 1000$.
\end{itemize}
%We computed the number of similar pairs by proposed algorithm for various real datasets;
%the largest instance, as-skitter, has $|V| = 1,696,145$ vertices and $|E| = 11,095,298$ edges.
The result is shown in Table~\ref{tbl:scalability},
which is the main result of this paper.
Here, ``dataset'', ``$|V|$'', and ``$|E|$'' denote the statistics of dataset,
``low'' and ``high'' denote the size of $J_L$ and $J_H$ in \eqref{eq:JLJH},
``estimate'' denotes the number of similar pairs estimated by the algorthm,
``filter'' and ``verification'' denotes the real time to compute filter and verification step,
and ``memory'' denotes the used memory.

This shows the proposed algorithm is very scalable.
In fact, for the network with 1M vertices and 10M edges,
the algorithm computes the number of similar pairs in 
30 minutes with 250 GB memory.



\subsection{Accuracy}

Next, we verify the accuracy (and the correctness) of the proposed algorithm.
We first compute the exact SimRank scores $S^*$ by using the original SimRank algorithm (Algorithm~\ref{alg:originalsimrank}).
Then, we compare the exact scores with the solution obtained by the proposed algorithm.
Here, the accuracy of the solution is measured by the precision, the recall, and the F-score~\cite{baeza1999modern}, defined by
\begin{align*}
  \text{precision} = \frac{|S \cap S^*|}{|S|}, \ 
  \text{recall}    = \frac{|S \cap S^*|}{|S^*|}, \ 
  \text{F}         = \frac{2 |S \cap S^*|}{|S|+|S^*|}.
\end{align*}
We use the same parameters shown in previous subsection for the proposed algorithm.
Since all-pairs SimRank computation is expensive, 
we used relatively small datasets for this experiment.

The result is shown in Table~\ref{tbl:accuracy}.
This shows the proposed algorithm is very accurate; 
the obtained solutions have about $\text{precision} \approx 97\%$, $\text{recall} \approx 92\%$, and $\text{F-score} \approx 95\%$.
We can observe that the proposed algorithm is conservative, i.e., 
pairs obtained by the proposed algorithm is really similar.

\begin{table}[tb]
\caption{Accuracy of algorithm.}
\label{tbl:accuracy}
\centering
\input{tbl_accuracy}
\end{table}


\subsection{Comparison with existing algorithms}


We then compare the proposed algorithm and some existing algorithms.
For the proposed algorithm, we used the same parameters described in the previous section.
For the existing algorithms, we implemented the following two algorithms%
\footnote{
We have also implemented the Sun et al.~\cite{sun2011link}'s LS-join algorithm;
however, it did not return a solution even for the smallest instance (ca-GrQc).
The reason is that their algorithm is optimized to find the top-$k$ (with $k \le 100$) similar pairs between given two small sets.}:
\begin{enumerate}
  \item Yu et al.~\cite{yu2010taming}'s all-pairs SimRank algorithm.
    We combine a thresholding heuristics that discard a small values in the SimRank matrix for each itereation.
    The algorithm runs in $O(n m)$ time with $O(n^2)$ memory. 
    For the SimRank join, We first compute the all-pairs SimRank by this algorithm and then count the number of similar pairs.

  \item Fogaras and Racz~\cite{fogaras2005scaling}'s random-walk based single-source SimRank algorthm.
    We set the number of Monte-Carlo samples $R = 1000$.
    We perform single-source SimRank computations for all seed vertices and then count the similar pairs.

%  \item Sun et al.~\cite{sun2011link}'s LS-join algorithm. It runs in $O(n m)$ time with $O(1)$ memory.
\end{enumerate}
We used three small datasets and three medium datasets.
For small datasets, we also compute the exact SimRank scores
and evaluate the accuracy.
For medium datasets, we only compare the scalability.

The result is shown in Table~\ref{tbl:comparison};
it shows the computational time for each dataset.
If an algorithm do not allocate memory in 256 GB environment, 
or requires about 2000 seconds, the result does not displayed.
This implies that the proposed algorithm is much efficient than
existing algorithms.

\begin{table}[tb]
\caption{Comparison of algorithms.}
\label{tbl:comparison}
\centering
\input{tbl_comparison}
\end{table}


\subsection{Experimental analysis of the algorithm}

In the previous subsections,
we observed that the proposed algorithm is 
scalable, accurate, and outperforms the existing algorithms.
In this subsection,
we evaluate the behavior of the algorithm.

We first evaluate the dependence with the accuracy parameter $\gamma$
used in \emph{filter} phase.
We vary $\gamma$ and compute the lower set $J_L$ and the upper set $J_H$.
The result is shown in Table~\ref{tbl:gamma}
This shows, to obtain an accurate upper and lower sets, 
we need to set $\gamma \ge 0.9$. 
However, it requires $10$ times longer computational time
and $10$ times larger memory.

\begin{table}[tb]
\caption{Dependency of accuracy parameter $\gamma$.}
\label{tbl:gamma}
\centering
\input{tbl_gamma}
\end{table}

Next, we evaluate the memory-reducing technique.
We vary the parameter $p$ and evaluate the used memory.
The result is shown in Table~\ref{tbl:memory_reducing}.
The column for $p = \infty$ shows the result without this technique.
Thus we compare other columns with this column.
The result shows that the effect of memory-reducing technique
greatly depends on the network structure.
However, for an effective case, it reduces memory about $1/2$.
By setting $p = 100$, we can obtain the same result as
the result without the technique.

\begin{table}[tb]
\caption{Dependency of the parameter $p$ for memory reducing technique.}
\label{tbl:memory_reducing}
\centering
\input{tbl_memory_reducing}
\end{table}

Finally, we evaluate the efficiencly improvement 
of our Monte-Carlo algorithm in \emph{verification} phase.
Since the proposed algorithm adaptively control the number of Monte-Carlo samples,
we show the average number of required number of samples.

\begin{table}[tb]
\caption{Average number of required samples.}
\label{tbl:required_samples}
\centering
\input{tbl_required_samples}
\end{table}


\section{Applications}

In this section, we demonstrate the proposed algorithm in some applications.


\subsection{Near duplication detection}

As mentioned in Introduction, the fundamental application of the similarity join query is the near-duplicate detection problem.
Here, we demonstrate the proposed algorithm in this application.

We use web-NotreDame dataset, which represents a web-graph in University of Notre Dame. 
The network consists of $281903$ vertices and $2312497$ edges;
see \cite{albert1999internet} for details of this dataset.
%
We construct a network as follows:
We randomly select 28190 ($10\%$) vertices, and clone these vertices with these links.
The obtained network $\tilde G$ consists of 310093 (=281903+28190) vertices.
The task is to detect these cloned vertices from the network.

We compute SimRank join for the reversed graph $\tilde G^\top$ with various threshold $\theta$.
The result is shown in Table~\ref{tbl:duplicate}. 
We obtained $XXX$ similar pairs candidate, and it contains all cloned vertices. 

\begin{table}[tb]
\caption{Near duplicate detection.}
\label{tbl:duplicate}
\centering
\input{tbl_duplicate}
\end{table}



\subsection{Number of similar pairs}

Cai et al.~\cite{cai2009efficient} claimed that 
the SimRank scores of a network follows power-law distributions.
However, they only verified this claim in small networks (at most 10000 vertices).

We here verify this conjecture in more larger networks.
We compute the number of similar pairs
by varing the similarith threshold $\theta$.
The result is shown in Figure~\ref{fig:number_of_similar_pairs}.
This shows, for each experimented dataset,
the number of similar pairs follows power law distributions.

%\begin{table}[tb]
%\caption{Number of similar pairs.}
%\label{tbl:number_of_similar_pairs}
%\centering
%\input{tbl_number_of_similar_pairs}
%\end{table}

\begin{figure}[tb]
\input{fig_similarpairs}
\caption{The number of similar pairs.}
\label{fig:number_of_similar_pairs}
\end{figure}


%% vim:foldmethod=marker


==> icde/verification.tex <==
\section{Verification phase}
\label{sec:verification}

In the previous section, we described the filter phase for enumerating the similar-pair candidates.
In this section, we discuss the verification phase for deciding whether each candidate $(i,j)$ is actually similar.
It should be mentioned that this procedure for each pair can be performed in parallel, i.e.,
if there are $M$ machines, the computational time is reduced to $1/M$.

Our verification algorithm is a \emph{Monte-Carlo algorithm}
based on the representation of the first meeting time~\eqref{eq:randomwalker}.
$R$ samples of the first meeting time $\tau^{(1)}(i,j), \ldots, \tau^{(R)}(i,j)$ are obtained from $R$ random walks
and the SimRank score is then estimated by the sample average:
\begin{align}
\label{eq:sampleaverage}
  s(i,j) \approx s^{(R)}(i,j) := \frac{1}{R} \sum_{k=1}^R c^{\tau^{(k)}(i,j)}.
\end{align}
To accurately estimate $s(i,j)$ by \eqref{eq:sampleaverage},
many samples (i.e., $r \ge 1000$) are required~\cite{fogaras2005scaling,maehara2014efficient}.
%However, whether $s(i,j)$ is greater than or smaller than the threshold $\theta$, it can be determined from much fewer samples.
However, to decide whether $s(i,j)$ is greater than or smaller than the threshold $\theta$, much fewer samples are required.
\begin{proposition}
\label{prop:hoeffding}
Let $\delta^{(R)} = |s^{(R)}(i,j) - \theta|$.
If $s(i,j) \ge \theta$ then
\begin{align}
  \P\{ s^{(R)}(i,j) < \theta \} \le \exp\left( - 2 R \delta^{(R) 2} \left(\frac{1-c}{c}\right)^2 \right).
\end{align}
Similarly, if $s(i,j) \le \theta$ then
\begin{align}
  \P\{ s^{(R)}(i,j) > \theta \} \le \exp\left( - 2 R \delta^{(R) 2} \left(\frac{1-c}{c}\right)^2 \right).
\end{align}
\end{proposition}
The proof will be given in Appendix. 
This shows that, if $s(i,j)$ is far from the threshold $\theta$,
it can be decided with a small number of Monte-Carlo samples.

Now we describe our algorithm.
We optimize the number of Monte-Carlo samples,
by adaptively increasing the samples.
%We start from $R = 1$ sample and repeating the following procedure.
Starting from $R = 1$, our verification algorithm loops through the following procedure.
The algorithm obtains $s^{(R)}(i,j)$ by performing
two random walks and computing $\tau^{(R)}(i,j)$.
It then checks the condition
\begin{align}
\label{eq:termination}
  R \delta^{(R) 2} \ge \frac{\log(1/p)}{2} \left( \frac{c}{1-c} \right)^2,
\end{align}
where $p \in (0,1)$ is a tolerance probability for misclassification.
If this condition is satisfied, we determine $s(i,j) < \theta$ or $s(i,j) > \theta$,
The misclassification probability of this decision is at most $p$
by Proposition~\ref{prop:hoeffding}.

\begin{algorithm}[tb]
\caption{Verification procedure.}
\label{alg:verification}
\begin{algorithmic}[1]
\Procedure{Verification}{$i$, $j$; $\theta$, $p$, $R_\mathrm{max}$}
\For{$R = 1, \ldots, R_{\mathrm{max}}$}
\State{Perform two independent random walks to obtain the first meeting time $\tau^{(r)}(i,j)$.}
\State{$s^{(R)} = (1/R) \sum_{k=1}^R \tau^{(k)}(i,j)$.}
\State{$\delta^{(R)} = |s^{(R)} - \theta|$.}
\If{$R \delta^{(R) 2}$ is large, i.e., \eqref{eq:termination} holds}
\State{\textbf{break}}
\EndIf
\EndFor
\If{$s^{(R)} \le \theta$}
\State{\Return $s(i,j) \ge \theta$}
\Else
\State{\Return $s(i,j) \le \theta$}
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

We now evaluate the number of samples required in this procedure.
By taking expectation of \eqref{eq:termination}, we obtain
the expected number of iterations $R_{\mathrm{end}}$ as
\begin{align}
  \E[ R_\textrm{end} ] \ge \frac{1}{(s(i,j) - \theta)^2} \frac{\log(1/p)}{2} \left( \frac{c}{1-c} \right)^2,
\end{align}
This shows that the number of samples quadratically depends on the inverse of the difference between the score $s(i,j)$ and the threshold $\theta$.
%Algorithm~\ref{alg:verification} can efficiently check $s(i,j) \le \theta$ or $s(i,j) \ge \theta$.
%However, if $s(i,j)$ is close to $\theta$, Algorithm~\ref{alg:verification} is very expensive.
In practice, we set an upper bound $R_\mathrm{max}$ of $R$, and
terminate the iterations after $R_\mathrm{max}$ steps.
Our verification algorithm is shown in Algorithm~\ref{alg:verification}.

%In Section~\ref{sec:experiments},
%we experimentally verified that
%the number of samples is about $100$.
%for a real network and $\theta = 0.2$,


==> kdd/abstract.tex <==
\begin{abstract}
SimRank, proposed by Jeh and Widom, provides a good similarity measure that has been successfully used in numerous applications.
While there are many algorithms proposed for computing SimRank,
their computational costs are very high.

In this paper, we propose a framework for computing SimRank accurately.
Our framework is based on the novel technique, \emph{linearized SimRank},
which provides efficient algorithms for
the single-pair, single-source, and all-pairs SimRank problems, respectively.
More specifically, our framework consists of two phases, a preprocessing phase and a query phase.
In the preprocessing phase, we estimate a parameter for a given graph and a desired accuracy by Monte Carlo simulation,
and then in the query phase,
we efficiently solve SimRank problems using this preprocessed parameter.
Our algorithms are efficient in both time and space.
The preprocessing phase is performed in nearly linear time
and the query phase requires only linear time for single-pair and single-source problems;
furthermore, the space complexity is linear for both preprocessing and query phase.

We conducted experiments to evaluate our algorithms.
For small networks ($n \le 1,000,000$), our algorithm required only a few minutes for preprocessing,
and then answered single-pair and single-source queries in 100 and 300 milliseconds, respectively.
All-pairs computation was performed in a few days.
For large networks ($n \ge 40,000,000$), our algorithm required a few hours for preprocessing, and
then answered single-pair and single-source queries approximately in 10 seconds and in a half minutes, respectively.

In comparison to previous studies,
for the all-pairs problem, our algorithm uses significantly less memory
than any existing algorithm; thus it scales for much larger networks. For the single-pair and the single-source problems,
our algorithm requires much fewer random samples than any existing
Monte Carlo based algorithm for the same accuracy solution.
\end{abstract}


==> kdd/conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}

In this paper, we propose a framework for computing SimRank
that is based on a linearized SimRank.
Our framework consists of two phases, a preprocessing phase and a query phase.
Once the preprocessing completes,
we can efficiently solve single-pair, single-source, and all-pairs SimRank problems.

Our experiments show that
our algorithm is fast and uses relatively low memory;
thus it can scale up to very large networks.
%By comparing existing algorithms,
%%very efficient algorithm for SimRank computation.
%Our algorithm is a two-phase method that estimates the parameters in preprocessing phase
%and computes SimRank scores in the query phase.
%We conducted our experiments to implement our proposed algorithm.
%The algorithm is accurate and scales up to the real networks of $n \ge 40,000,000$,
%and it is 1000 times faster than the existing results.

For future work,
it would be interesting to extend our method to dynamic networks~\cite{LHHJSYW10}.
When a network is modified by adding or removing vertices or edges,
we must efficiently update matrix $D$.
%estimated parameters efficiently.
Establishing such a method will be noteworthy both in theory and practice.

In general,
our linearization technique can be applied to
recursively defined values with a maximum. %that are recursively defined with maximum.
For example,
consider P-Rank~\cite{ZHS09,CC11},
which generalizes SimRank as follows.
Let $P$ be a transition matrix of $G^\top$ and let $Q$ be a transition matrix of $G$.
Then P-Rank is defined by
\[
S = \left( (1 - \lambda) c P^\top S P + \lambda c Q^\top S Q \right) \lor I.
\]
SimRank is the case in which $\lambda = 0$, and rvs-SimRank~\cite{ZHS09} is the case in which $\lambda = 1$;
i.e., SimRank only uses the in-link information,
whereas rvs-SimRank only uses out-link information,
but P-Rank uses both types of links.
We can establish a linear formulation of P-Rank as
$$ S = \left( (1 - \lambda) c P^\top S P + \lambda c Q^\top S Q \right) + D $$
with a suitable diagonal matrix $D$.
Therefore we can possibly extend our algorithm to P-Rank by the above formula.


==> kdd/contribution.tex <==
\subsection{Contribution}

In this paper, we propose a framework for efficiently computing SimRank
with an arbitrary accuracy $\epsilon$ (i.e., the error is less than $\epsilon$).
Our framework consists of two phases, a \emph{preprocessing phase} and a \emph{query phase}.
In the preprocessing phase, we estimate a diagonal matrix $D$, which is defined in Section~\ref{sec:LinearizedSimRank} and which plays a crucial role in our framework, for a given graph and an accuracy $\epsilon$,
and in the query phase, by using this estimated matrix $D$,
we solve single-pair, single-source, and all-pairs SimRank problems.
%
The obtained algorithms are efficient in both time and space, as described below.
% TODO: accuracy

%\begin{description}
%\item[Efficient in time]
\medskip
\noindent \textbf{Efficient in time.} \quad
The preprocessing phase to estimate a matrix $D$
is an iterative algorithm with Monte Carlo simulation
(Subsections~\ref{sec:Alternating} and~\ref{monte}).
The time complexity of this phase is $O(T L R n)$,
where $T$ is the number of iterations to compute SimRank scores,
$R$ is the number of Monte Carlo samples,
and $L$ is the number of iterations for the estimation algorithm.
It can be shown that 
%The latter two values can be mathematically shown as follows: 
$R = O((\log n)/\epsilon^2)$ and
$L = O(\log (n/\epsilon))$ (Subsection~\ref{sec:accuracy}).
%where $\epsilon$ is the desired accuracy.
Thus, the time complexity is expected to be nearly linear.
Note that the preprocessing phase is the most computationally intensive part of our framework.

Once this matrix $D$ is estimated,
SimRank scores can be computed by deterministic algorithms (Section~\ref{sec:LinearizedSimRankComputation}).
The single-pair problem can be solved in $O(T m)$ time,
the single-source problem can be solved in $O(T^2 m)$ time,
and the all-pairs problem can be solved in $O(T^2 n m)$ time
by solving single-source problems for all vertices.
Note that our all-pairs algorithm can easily be parallelized to
multiple machines, i.e.,
if we have $M$ machines, it can run in $O(T^2 n m / M)$ time.
%Thus it can scale up to a large graph.

%\item[Efficient in space.]
\medskip
\noindent \textbf{Efficient in space.} \quad
In both the preprocessing and query phases,
the algorithms only require $O(n)$ extra space to store a diagonal matrix $D$ and vectors of length $n$.
thus the total space complexity is $O(m)$.
%which is only used to store the input network.
Note that for the all-pairs case, we do not have to \emph{store} the similarity of all pairs of vertices.
We emphasize that
this is the first linear space algorithm to compute all-pairs SimRank scores.
%
%\end{description}

\medskip

We evaluated our algorithms using real networks in Section~\ref{sec:Experiments}.
For small networks ($n \le 1,000,000$),
our algorithm took only a few minutes for preprocessing,
and then answered single-pair and single-source queries in 100 and 300 milliseconds (on average), respectively.
All-pairs computation was performed in a few days.
For large networks ($n \ge 40,000,000$), our algorithm required a few hours for preprocessing,
and then answered single-pair and single-source queries approximately in 10 seconds and in a half minutes (on average), respectively.
To the best of our knowledge, our experiment is performed on the largest datasets in the literature.

%We also compare our algorithm with the existing ones in Subsection~\ref{sec:Comparison}.
% TODO: compare

\medskip
\noindent \textbf{Comparison with other existing algorithms.} \quad
We compare our algorithm with the existing ones in Subsection~\ref{sec:Comparison}.
%As a result,
%In comparison to previous studies,
Our algorithms have the following advantages:
\begin{enumerate}
\item
The state-of-the-art all-pairs algorithm, proposed by Yu et al.~\cite{YZLZL12}, requires much more memory, and hence works only for small networks which has $n \le$ 1,000,000 vertices.
On the other hand,
our algorithm requires much less memory,
therefore it works for a very large networks.
%than the existing all-pairs algorithms, such as Yu et al.~\cite{YZLZL12},
%and hence our algorithm works for a larger networks than their algorithm.
%(Note that the existing algorithm only worked for $n < 1,000,000$ networks).
%Furthermore, our all-pairs algorithm can easily be parallelized to multiple machines;
%thus it scales well.

\item
%In order
%to obtain the same accuracy solution,
The state-of-the-art Monte Carlo based single-pair and single-source algorithm by Fogaras and Racz~\cite{FR05} also requires much more space. 
%random samples than our
%algorithm (e.g., their algorithm requires $R' \ge$ 100,000 samples
%for the same accuracy solution of our algorithm with $R = 100$ samples).
%Thus, to compute SimRank scores accurately,
%our algorithm is much faster and uses much less space than their algorithm.
\end{enumerate}


%Technically speaking,
Our framework is based on a novel technique, named \emph{linearized SimRank}.
In Section~\ref{sec:LinearizedSimRank},
we observe that the computational difficulty of SimRank comes from its \emph{non-linearity}.
We introduced linearized SimRank to overcome this difficulty,
which enabled us to compute SimRank scores via a \emph{linear recurrence equation}.


\subsection{Organization}

In Section~\ref{sec:LinearizedSimRank}, we introduce the linearized SimRank,
which is the main idea of our paper.
In Section~\ref{sec:LinearizedSimRankComputation},
we propose algorithms for three fundamental problems for SimRank, which are based on the linearized SimRank.
In Section~\ref{sec:DiagonalEstimation},
we propose a parameter estimation algorithm, which is required for preprocessing.
In Section~\ref{sec:Experiments},
we evaluate our algorithm on several real networks
in terms of accuracy and efficiency.
We also give comparisons with existing algorithms.
Finally in Section~\ref{sec:Conclusion},
we conclude our paper and describe future work.



==> kdd/introduction.tex <==
\section{Introduction}

\subsection{SimRank}

In recent years, much effort has been devoted to extracting useful information from large graphs.
With the rapidly increasing amount of graph data, 
the \emph{similarity search problem}, which identifies similar vertices in a graph,
has become an important problem
with many applications, including 
web analysis~\cite{JW02,LK07},
graph clustering~\cite{YHY06,ZCY09},
spam detection~\cite{GGP04},
computational advertisement~\cite{AMC08},
recommender systems~\cite{AM07,YSY10},
and 
natural language processing~\cite{C10}.

Several similarity measures have been proposed~\cite{Kes63,Sma73,LKL06,LLK07,LLK12}.
In this paper, we focus on \emph{SimRank}~\cite{JW02}.
SimRank is a link-based similarity measure proposed for similarity searches on the World Wide Web.
The fundamental idea behind SimRank is that
\begin{quote}
two pages are similar if they are referenced by similar pages.
\end{quote}
This intuition is formulated as follows.
Let $G = (V, E)$ be a directed graph with vertex set $V = \{1, \ldots, n\}$.
\emph{SimRank} $s(i,j)$ of vertex $i$ and $j$ is recursively defined by
\begin{align}
\label{eq:DefinitionOfSimRankEntrywise}
s(i,j) = \begin{cases}
1, & (i = j), \\
\displaystyle \frac{c}{|\In(i)| |\In(j)|} \sum_{\substack{i' \in \In(i), j' \in \In(j)}} s(i',j'), & (i \neq j),
\end{cases}
\end{align}
where $\In(i) = \{ j \in V : (j,i) \in E\}$ is the set of in-neighbors of $i$,
and $c \in (0,1) $ is a decay factor usually set to $c = 0.8$~\cite{JW02} or $c = 0.6$~\cite{LVGT08}.
%
%
%
SimRank and its related measures~\cite{AMC08,CLLHD08,ZHS09,YLZCP13}
%(e.g., SimRank++~\cite{AMC08},  S-SimRank~\cite{CLLHD08}, P-Rank~\cite{ZHS09}, SimRank$^*$~\cite{YLZCP13}, etc)
give high-quality scores in many application areas,
because it takes multi-step neighborhoods into account,
whereas other similarity measures, such as the Jaccard coefficient,
utilize only one-step neighborhoods.
%This is a similar reason for PageRank, as used by the Google search engine, because both SimRank and PageRank can
%take global information of given networks into account.
%Indeed, both can be defined as the ``random surfer-pairs
%model''.

While there are several algorithms proposed to compute SimRank scores, 
its computation cost is very high.
More precisely, there are three fundamental SimRank problems:
\begin{description}
  \item[Single-pair SimRank.] Given two vertices $i, j \in V$, compute SimRank score $s(i,j)$.
  \item[Single-source SimRank.] Given a vertex $i \in V$, compute SimRank scores $s(i,j)$ for all $j \in V$.
  \item[All-pairs SimRank.] Compute SimRank scores $s(i,j)$ for all $i, j \in V$.
\end{description}
Most existing algorithms solve the all-pairs SimRank problem using $O(n^2)$ space, where $n$ is the number of vertices;
thus they are impractical for large graphs.
%The fastest existing method is performed for a graph, which has three million vertices and 16 million edges, in 39 hours~\cite{YLZCP13}.
A few algorithms solve the single-pair and single-source problems, but they also have accuracy and complexity issues, which we describe in Section~\ref{sec:Comparison}.
%Furthermore, to the best of our knowledge,
%there is no efficient algorithm for the single-source SimRank problem.

Therefore, the purpose of this paper is to propose efficient algorithms, 
in both time and space, for these SimRank problems.


==> kdd/notation.tex <==
%\section{Notations}
%
%$G = (V, E)$ denotes a directed graph.
%$n = |V|$ and $m = |E|$.
%$G^\top = (V, E^\top)$ denotes a transpose graph of $G$, i.e,
%$(i,j) \in E^^top$ if $(j,i) \in E$.
%$\delta_-(i)$ denotes a set of in-links of $i$.
%
%$P$ denotes a transition matrix of $G^\top$, i.e.,
%$$ P_{ij} = \begin{cases} 1 / \delta_-(j) & (i,j) \in E^\top,
%\\ 0 & \textrm{otherwise}. $$
%

%\begin{table}
%\caption{Frequenty-used notations}
%\begin{center}
%\begin{tabular}{ll}
%Notation & Definition and Description \\ \hline
%$G = (V,E)$ & A directed graph \\
%$G^\top$ & Transposed graph of $G$ \\
%$n$ & The number of vertices of $G$ \\
%$m$ & The number of edges of $G$ \\
%$\delta_-(i)$ & Set of in-links of $i$ \\
%$P$ & Transition matrix of $G^\top$ \\
%$S$ & SimRank matrix \\
%$S^L(\Theta)$ & Linearized SimRank matrix \\
%$\Theta$ & Correction matrix \\
%$D$ & The diagonal estimation \\
%$T$ & The number of SimRank iteration \\
%\end{tabular}
%\end{center}
%\end{table}


==> kdd/parameter.tex <==


%%% OBSOLETE %%%

\section{Parameter selection}
\label{sec:ParameterSelection}

%Both SimRank and our algorithm have the following four parameters:
SimRank and our algorithm have the following four parameters:
(1) $c$, the decay factor of SimRank,
(2) $T$, the number of iterations of SimRank,
(3) $L$, the number of outer-loops of Algorithm~\ref{alg:DiagonalEstimation},
and
(4) $R$, the number of samples of Monte Carlo simulation in Algorithm~\ref{alg:DiagonalUpdate}.
We here discuss the suitable setting of these values.
To be concrete, we suppose that
we want to compute the SimRank score with accuracy less than $\epsilon = 0.01$.

\subsection*{Decay factor / Number of iterations}

For the original SimRank,
%Note that, the similar analsis for SimRank is given by Lizorkin et al.~\cite{LVGT08}.
Jeh and Widom~\cite{JW02} suggested using $c = 0.8$ and $T = 5$,
but recently, Lizorkin et al.~\cite{LVGT08} pointed out 
that these parameters could cause (numerically) inaccurate solutions.
They suggested using either a small decay factor (e.g., $c = 0.6$) or more iterations.

We here set the decay factor $c = 0.6$.
We can show that, the approximation error of $T$-th iterated solution is $c^T/(1-c)$
(see Proposition~\ref{prop:ConvergenceNeumann} and Proposition~\ref{prop:DisNonnegative}).
Hence, we set $T = 11$ in order for $c^T/(1-c) \le 0.01$.

\subsection*{Number of outer-loops / Number of samples}

We next discuss the number of outer-loops $L$ and the number of samples $R$.
In the previous section, we analyzed $L = O(\log(1/\epsilon) / \log d)$ and $R = O(\log n / \epsilon^2)$.
However, since the theoretical analysis is for the worst case,
we can use much smaller values in practice.
To compute SimRank in large networks efficiently,  
this is an important optimization.

To optimize the parameters, 
we empirically evaluates the accuracy of the algorithm.
We first compute the ``exact'' SimRank scores, $s_{\textrm{exact}}$, by the original algorithm by Jeh and Widom~\cite{JW02}.
We then compute SimRank score, $s_{\textrm{proposed}}$, by our algorithm, and compare these values in the maximum difference of off diagonal scores:
\[
  \textrm{error} = \max_{i \neq j} | s_{\textrm{exact}}(i,j) - s_{\textrm{proposed}}(i,j) |.
\]
Since the above evaluation requires heavy computation,
we here use three (small) datasets: ``as20000102'' dataset~\cite{LKF05}, ``ca-GrQc'' dataset~\cite{LKF05}, and ``wiki-Vote'' dataset~\cite{LHK10-1,LHK10-2}.
The results are shown in Figures~\ref{fig:accuracy}.

We can observe that
\begin{itemize}
\item The proposed algorithm can compute SimRank with high accuracy.
\item The number of iterations $L$ is enough for $3$ to $5$.
\end{itemize}

\begin{figure}[ht]
  \centering
  \subfloat[as20000102]{\epsfig{file=figure/as20000102.eps, width=13em}}
  \subfloat[ca-GrQc]{\epsfig{file=figure/ca-GrQc.eps, width=13em}}
%  \subfloat[wiki-Vote]{\epsfig{file=figure/wiki-Vote.eps, scale=0.60, bb=50 0 260 160}}
  \caption{Number of iterations $L$ vs. absolute error} \label{fig:accuracy}
\end{figure}


%
%\begin{table}[ht]

%
%The tight convergence analysis of the Algorithm~\ref{alg:DiagonalEstimation} is difficult.
%Hence we here use the numerical simulation
%to decide the suitable number $L$.
%
%We use ``as20000102'' dataset~\cite{LKF05}, ``ca-GrQc'' dataset~\cite{LKF05}, and ``wiki-Vote'' dataset~\cite{LHK10-1,LHK10-2}.
%``as20000102'' dataset is a communication network of autonomous systems,
%``ca-GrQc'' dataset is a collaboration network obtained from e-print arXiv,
%and
%``wiki-Vote'' dataset is a voting network of an administrator election of Wikipedia.
%
%We apply our diagonal estimation algorithm for these networks
%and plot the convergence curve.
%We here measure the accuracy by the mean squared error of the diagonal elements,
%i.e., $\sqrt{ \sum_i (1 - S^L(D)_{ii})^2 }$.
%The results are shown in Figure~\ref{fig:accuracy}.
%
%We can observe that
%the convergence curve depends on graphs and the number of samples, but
%a few (e.g., two or three) iterations are sufficient for convergence.
%Hence we set $L = 2$.
%
%XXX
%
%\begin{figure}[!h]
%  \centering
%  \subfloat[as20000102]{\epsfig{file=figure/as20000102.eps, scale=0.60, bb=50 0 260 160}}
%  \subfloat[ca-GrQc]{\epsfig{file=figure/ca-GrQc.eps, scale=0.60, bb=50 0 260 160}}
%
%  \subfloat[wiki-Vote]{\epsfig{file=figure/wiki-Vote.eps, scale=0.60, bb=50 0 260 160}}
%  \caption{Number of iterations $L$ vs. mean squared error of diagonals} \label{fig:accuracy}
%\end{figure}
%
%
%\subsection*{Number of samples of Monte Carlo simulation}
%
%To figure out a suitable number $R$,
%we plot the number of samples versus the mean squared error of diagonals.
%We conducted our experiment for three networks used above.
%The result is shown in Figure~\ref{fig:accuracy2}.
%We can observe that the mean squared error of diagonals is $O(1/R)$.
%Hence we set $R = 30$, because the mean squared error for all the three networks is about $10^{-3}$.
%\begin{figure}[!h]
%\centering
%  \epsfig{file=figure/sample-vs-error.eps, scale=0.60, bb=50 0 260 160}
%  \caption{Number of samples $R$ vs. mean squared error of diagonals} \label{fig:accuracy2}
%\end{figure}
%
%
%\subsection*{Justification of parameters}
%
%Now we propose the parameters $c = 0.6$, $T = 11$, $L = 2$, and $R = 30$.
%We here empirically justificate these parameters on small networks.
%
%We first compute the ``exact'' SimRank scores by the original algorithm proposed by Jeh and Widom~\cite{JW02}.
%We then compute SimRank score by our algorithm, and compare these values in the maximum difference of off-diagonal scores, $\max_{i \neq j} | S_{\textrm{exact}}(i,j) - S_{\textrm{proposed}}(i,j) |$.
%
%\begin{table}[ht]
%\caption{Accuracy of proposed algorithm}
%\centering
%\begin{tabular}{rr|rrrrrr}
%    &       &   &   &   & $L$ & &  \\
%    &       & 0 & 1 & 2 & 3 & 4 & 5  \\ \hline 
%    & 10    & 0.355 & 0.127 & 0.125 & 0.131 & 0.128 & 0.118 \\
%$R$ & 100   & 0.355 & 0.060 & 0.028 & 0.131 & 0.128 & 0.118 \\
%    & 1000  & 0.355 & 0.060 & 0.028 & 0.131 & 0.128 & 0.118 \\
%    & 10000 & 0.355 & 0.060 & 0.028 & 0.131 & 0.128 & 0.118 \\
%\end{tabular}
%\end{table}


==> kdd/relatedwork.tex <==
\subsection{Related work}

In this subsection,
we review existing algorithms for SimRank computation.
%There are known algorithms for the all-pairs and the single-pair problems.

\paragraph{All-pairs SimRank}

In the original paper by Jeh and Widom~\cite{JW02},
SimRank is computed by recursively evaluating
equation \eqref{eq:DefinitionOfSimRankEntrywise} for all $i, j \in V$.
This naive computation yields an $O(T m^2)$ time algorithm,
where $m$ denotes the number of edges, and $T$ denotes the number of iterations.
Lizorkin et al.~\cite{LVGT08} proposed a \emph{partial sum} technique to reduce the
time complexity to $O(T \min \{n m, n^3 / \log n \} )$.
Jia et al.~\cite{JLZHD10} removed dangling vertices, which are vertices with no in-links,
since the SimRank scores of these vertices are always zero.
Yu et al.~\cite{YZLZL12} introduced a matrix-based iteration approach
and applied a fast matrix multiplication algorithm~\cite{S69,W12}
that yields an $O(T \min \{n m, n^\omega \} )$ time algorithm,
where $\omega < 2.373$ is the exponent of matrix multiplication.
Cai et al.~\cite{CCJLHLD09} proposed an algorithm that discards
SimRank scores less than a predefined threshold,
a technique already employed in previous algorithms~\cite{LVGT08,YZLZL12}.
They showed that this technique works effectively on scale-free networks.
Jia et al.~\cite{JCLHD09} proposed an algorithm to maintain only vertex pairs of small distances
and showed that
this technique works effectively on small-world networks.

We emphasize that for all existing algorithms for the all-pairs problem,
the space complexity of these algorithms is $O(n^2)$,
since they must maintain all SimRank scores for each pair of nodes
to evaluate equation \eqref{eq:DefinitionOfSimRankEntrywise}.

\paragraph{Single-pair SimRank}

Jeh and Widom~\cite{JW02} provided a random-walk
interpretation of SimRank, called a \emph{random surfer pair model}.
Consider two random walks that start from vertices $i$ and $j$ respectively,
and follow their in-links.
Let $\tau(i,j)$ be the random variable that denotes the first meeting time of $i$ and $j$.
Then the SimRank score is obtained by
\begin{align} \label{eq:SimRankFirstMeetingTime}
s(i,j) = \E[ c^{\tau(i,j)} ],
\end{align}
where $\E$ denotes the expectation.
Fogaras and R\'acz~\cite{FR05} evaluated the right hand side via
Monte Carlo simulation with a fingerprint tree data structure.
This requires $O(n R')$ space to maintain $R'$ random walks for each vertex,
and computes a SimRank score $s(i,j)$ in $O(T R')$ time.
Furthermore, they extended their method for single-source query
that simultaneously computes single-pair queries for (possibly) similar vertices
by traversing the fingerprint tree; this yields an $O(T R' n)$ time algorithm.
Li et al.~\cite{LLYHD10} also used the random surfer pair model,
but their algorithm is deterministic;
more specifically, their algorithm is an iterative algorithm for the first meeting time,
and requires $O(n^2)$ space.

\medskip

Note that some papers~\cite{FNSO13,LHHJSYW10,YLL10,YLZCP13} %,HFLC10}
proposed spectral decomposition (or low-rank decomposition) based algorithms;
however, unfortunately, their algorithms do not actually compute SimRank,
because their algorithms are based on an incorrect formula;
see Remark~\ref{rem:wrong} in Section~\ref{sec:LinearizedSimRank} below.



==> sigmod/abstract.tex <==
\begin{abstract}
%Much effort has been devoted to extracting useful information from large graphs
%in research community. Some successful examples show that
%vertex similarities play a central role in
%many applications: link prediction, graph clustering, spam detection, and recommender %systems.
SimRank, proposed by Jeh and Widom, provides a good similarity score and has been
successfully used in many of the above mentioned applications.
While there are many algorithms proposed so far to compute SimRank, but
unfortunately, none of them are scalable up to graphs of billions size.
Motivated by this fact, we consider the following SimRank-based similarity search problem:
given a query vertex $u$,
find top-$k$ vertices $v$ with the $k$ highest SimRank scores $s(u,v)$ with respect to $u$.
%

We propose a very fast and scalable algorithm for this similarity search problem.
Our method consists of the following ingredients:
\begin{enumerate}
  \item
    We first introduce a ``linear'' recursive formula for SimRank. This allows us to formulate a problem that we can propose a very fast algorithm.
%    In addition, this formulation is very convenient to analyze the correctness of our algorithm.
%
  \item
    We establish a Monte-Carlo based algorithm to compute a single pair SimRank score $s(u,v)$, which is based on the random-walk interpretation of our linear recursive formula. %The time complexity is constant, i.e, independent of $n$.
  \item
    We empirically show that SimRank score $s(u,v)$ decreases rapidly
    as distance $d(u,v)$ increases.
    Therefore, in order to compute SimRank scores for a query vertex $u$ for our similarity search problem,
    we only need to look at very ``local'' area.
  \item
    We can combine two upper bounds for SimRank score $s(u,v)$ (which can be obtained by Monte-Carlo simulation in our preprocess), together with some adaptive sample technique, to prune the similarity search procedure. This results in a much faster algorithm.
\end{enumerate}
%Our algorithm gives almost exact top-$k$ vertices.
%In addition our algorithm scales up to very large networks. Indeed,
Once our preprocess is done (which only takes
$O(n)$ time), our algorithm finds, given a query vertex $u$, top-20 similar vertices $v$ with the 20 highest SimRank scores $s(u,v)$ in less than a few seconds even for graphs with billions edges.
%We can also find, for all vertices of a given  millions size real network, top-100 %similar vertices with the 100 highest SimRank scores in reasonable computation time.

To the best of our knowledge, this is the first
time to scale for graphs with at least billions edges(for the single source case).
%Indeed, our algorithm scales nearly 70 times bigger graphs than
%any other existing algorithm.
\end{abstract}


==> sigmod/algorithm.old.tex <==
\section{Algorithm}
\label{sec:algorithm}

We are now ready to provide our whole algorithm.
Our algorithm consists of two phases: preprocess phase and query phase.

In the preprocess phase, we precompute $\gamma$ in \eqref{eq:gamma} for the L2 bound.
Note that we compute $\alpha,\beta$ in \eqref{eq:alpha}, \eqref{eq:beta} for L1 bound in query phase.
As described in Algorithm~\ref{alg:gamma},
it requires $O(n R T)$ time, where $R$ is the number of Monte-Carlo samples and $T$ is the length of random walks.

In the query phase, given a query vertex $u$ and rank $k$,
we compute the top-$k$ SimRank scores with respect to a query vertex $u$
in ascending order of distance from $u$ (this can be done by breadth first search).
By maintaining the SimRank scores by min-heap,
the query algorithm requires $O(n' \log k R T)$ time,
where $n'$ is the number of vertices in the ball of some (small) radius around $u$ that are examined in the algorithm.
In the worst case $n' = n$. However, in practice,
the radius is smaller than average distance of networks (as shown in Section~\ref{sec:correctness}. Indeed 
the radius would be at most three)
and hence $n'$ is much smaller than $n$.
Since every similar vertices are placed on distance  $3 \sim 5$ in practice,
we can expect $n' \sim d^{3 \sim 5}$ where $d$ is the average degree of the network.
Indeed, from our experiments given in Section~\ref{sec:experiment},
$n'$ seems to depend on the network structure (e.g., web graph or social network)
rather than the network size (i.e., $n$ and $m$).


\begin{algorithm}[ht]
\caption{Proposed algorithm (preprocess)}
\begin{algorithmic}[1]
\Procedure{Preprocessing}{}
\For{$u \in V$}
\State{Compute $\gamma(u)$ by Algorithm~\ref{alg:gamma}}
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[ht]
\caption{Proposed algorithm (query)}
\begin{algorithmic}[1]
\Procedure{Query}{$u$,$k$}
\State{$H \leftarrow$ empty min-heap sorted by $s(u,\cdot)$}
\For{$d = 1, 2, \ldots$}
\State{Compute $\alpha(u,d,t)$ by Algorithm~\ref{alg:alpha}}
\State{Compute $\beta(u,d)$ by \eqref{eq:beta}}
\If{$|H| = k$ and $\beta(u, d) \le s(u,H[k])$}
\State{\textbf{return} $H[1], \ldots, H[k]$}
\EndIf
\For{$v \in V$ with $d(u,v) = d$}
\If{$\sum_{t=0}^T c^t \gamma(u,t) \gamma(v,t) \le s(u,H[k])$}
\State{$\mathbf{continue}$}
\EndIf
\State{Compute $s(u,v)$ by Algorithm~\ref{alg:singlepair}}
\If{$s(u,v) > s(u,H[k])$}
\State{$\mathtt{push}(v, H)$}
\If{$|H| > k$}
\State{$\mathtt{pop}(H)$}
\EndIf
\EndIf
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> sigmod/algorithm.tex <==
\section{Algorithm}
\label{sec:algorithm}

We are now ready to provide our whole algorithm for top-$k$ similarity search.
Our algorithm consists of two phases: preprocess phase and query phase.
In the query phase, for a given vertex $u$,
we compute single-pair SimRanks $s(u,v)$ for some vertices $v$ that may have high SimRank value (we call such vertices \emph{candidates} that are computed in the preprocess phase), 
and output $k$ highly similar vertices.

In order to obtain similar vertices accurately,
we have to perform many Monte Carlo simulations
in single-pair SimRank computation (Algorithm~\ref{alg:singlepair}).
Thus, the key of our algorithm is the way to reduce the number of candidates that 
are computed in the preprocess phase in Section 7.1.

\subsection{Preprocess phase}

In the preprocess phase, we precompute $\gamma$ in \eqref{eq:gamma} for the L2 bound as described in Algorithm~\ref{alg:gamma}.
Note that we compute $\alpha,\beta$ in \eqref{eq:alpha}, \eqref{eq:beta} for the L1 bound in query phase.
%As described in Algorithm~\ref{alg:gamma},
%it requires $O(n R T)$ time, where $R$ is the number of Monte-Carlo samples and $T$ is the length of random walks.

After that, for each vertex $u$, we enumerate ``candidates'' of highly similar vertices $v$.
For this purpose, we consider the following auxiliary bipartite graph $H$.
The left and right vertices of $H$ are copy of $V$ (i.e., $H$ has $2 n$ vertices).
Let $u_\mathrm{left}$ be the copy of $u \in V$ in the left vertices and
let $v_\mathrm{right}$ be the copy of $v \in V$ in the right vertices.
There is an edge $(u_\mathrm{left}, v_\mathrm{right})$ if
a random walk that starts from $u$ frequently reaches $v$.
By this construction,
a pair of vertices $u$ and $v$ has high SimRank score if
$u_\mathrm{left}$ and $v_\mathrm{left}$ share many neighbors.
We construct this bipartite graph $H$ by performing Monte-Carlo simulations in the original graph $G$ as follows.
For each vertex $u$, we iterate the following procedure $P$ times
to construct an index for $u$.
We perform a random walk $W_0$ of length $T$ from $u$ in $G$.
We further perform $Q$ random walks $W_1, \ldots, W_Q$ from $u$.
Let $v$ be $t$-th vertex on $W_0$.
Then we put an edge $(u_\mathrm{left}, v_\mathrm{right})$ in $H$ if
there are at least two random walks in $W_1, \dots W_Q$ that contain $v$
at $t$-th step. The whole procedure is described in Algorithm 3 below.
Here, for a random walk $W_j$ and $t \ge 0$, we denote the vertex at the $t$-th step of $W_j$ by $W_{jt}$.

%
%We further perform $Q$ random walks from
%For each step,
%For each walk $W$,
%We perform $P$ random walks in $G$ for each vertex $u$.
%We further
%Then we put an edge $(u_\mathrm{left}, v_\mathrm{right})$ in $H$ if
%there are at least two random walks that contain the vertex $v$ at the same step $t$.

In our experiment, we set $P=10$, $T=11$ and $Q=5$.
The time complexity of this preprocess phase is $O(n (R + P Q) T)$,
where $R$ comes from Algorithm 3 and we set $R=100$ in our experiment.
The space complexity is $O(n P)$, but in practice,
since the number of candidates are usually small,
the space is less smaller than this bound.
%In the preprocess phase, we precompute $\gamma$ in \eqref{eq:gamma} for the L2 bound.
%Note that we compute $\alpha,\beta$ in \eqref{eq:alpha}, \eqref{eq:beta} for L1 bound in query phase.
%As described in Algorithm~\ref{alg:gamma},
%it requires $O(n R T)$ time, where $R$ is the number of Monte-Carlo samples and $T$ is the length of random walks.

\begin{algorithm}
\caption{Proposed algorithm (preprocess)}
\begin{algorithmic}[1]
  \Procedure{Indexing}{}
  \For{$u \in V$}
  \For{$i = 1, \ldots, P$}
    \State{Perform a random walk $W_0$ from $u$}
    \State{Perform random walks $W_1$,$\ldots$,$W_Q$ from $u$}
    \For{$t = 1, \ldots, T$}
      \If{$W_{jt} = W_{kt}$ for some $j \neq k$}
      \State{Add $W_{0t}$ for index of $u$}
      \EndIf
    \EndFor
  \EndFor
  \EndFor
  \EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Query phase}

%In the query phase, given a query vertex $u$ and rank $k$,
%we enumerate the top-$k$ SimRank scores with respect to a query vertex %$u$.

We now describe our query phase.
For a given vertex $u$, we first traverse the auxiliary bipartite graphs $H$
and enumerate all the vertices $v$ that share the neighbor in $H$.
We then prune some vertices $v$ by L1 and L2 bounds.
After that, for each candidate $v$,
we compute SimRank scores $s(u,v)$ by Algorithm~\ref{alg:singlepair}.
Finally we output top $k$ similar vertices as the solution of similarity search.

To accelerate the above procedure, we use the adaptive sample technique.
For a query vertex $u$,
we first set $R = 10$ (in Algorithm~\ref{alg:singlepair}) and 
estimate SimRank scores roughly for each candidate $v$
by Monte Carlo simulation
(i.e, we only perform 10 random walks for $v$ by Algorithm~\ref{alg:singlepair}).
Then, we change $R = 100$ and re-compute more accurate SimRank scores
for each candidate $v$ that has high estimated SimRank scores by Monte Carlo simulation (i.e, we perform
100 random walks for $v$ by Algorithm~\ref{alg:singlepair}).
The whole procedure is described in Algorithm 5.

The overall time complexity of the query phase is
$O(R T |S|)$ where $|S|$ is the number of candidates, since
computing  SimRank scores $s(u,v)$ by Algorithm~\ref{alg:singlepair} for
two vertices $u,v$ takes $O(RT)$.
The space complexity is $O(m + nP)$.

%in ascending order of distance from $u$ (this can be done by breadth first search).
%By maintaining the SimRank scores by min-heap,
%the query algorithm requires $O(n' \log k R T)$ time,
%where $n'$ is the number of vertices in the ball of some (small) radius around $u$ that are examined in the algorithm.
%In the worst case $n' = n$. However, in practice,
%the radius is smaller than average distance of networks (as shown in Section~\ref{sec:correctness}. Indeed
%the radius would be at most three)
%and hence $n'$ is much smaller than $n$.
%Since every similar vertices are placed on distance  $3 \sim 5$ in practice,
%we can expect $n' \sim d^{3 \sim 5}$ where $d$ is the average degree of the network.
%Indeed, from our experiments given in Section~\ref{sec:experiment},
%$n'$ seems to depend on the network structure (e.g., web graph or social network)
%rather than the network size (i.e., $n$ and $m$).

%
%\begin{algorithm}[ht]
%\caption{Proposed algorithm (preprocess)}
%\begin{algorithmic}[1]
%\Procedure{Preprocessing}{}
%\For{$u \in V$}
%\State{Compute $\gamma(u)$ by Algorithm~\ref{alg:gamma}}
%\EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%


%\begin{algorithm}[ht]
%\caption{Proposed algorithm (query)}
%\begin{algorithmic}[1]
%\Procedure{Query}{$u$,$k$}
%\State{$H \leftarrow$ empty min-heap sorted by $s(u,\cdot)$}
%\For{$d = 1, 2, \ldots$}
%\State{Compute $\alpha(u,d,t)$ by Algorithm~\ref{alg:alpha}}
%\State{Compute $\beta(u,d)$ by \eqref{eq:beta}}
%\If{$|H| = k$ and $\beta(u, d) \le s(u,H[k])$}
%\State{\textbf{return} $H[1], \ldots, H[k]$}
%\EndIf
%\For{$v \in V$ with $d(u,v) = d$}
%\If{$\sum_{t=0}^T c^t \gamma(u,t) \gamma(v,t) \le s(u,H[k])$}
%\State{$\mathbf{continue}$}
%\EndIf
%\State{Compute $s(u,v)$ by Algorithm~\ref{alg:singlepair}}
%\If{$s(u,v) > s(u,H[k])$}
%\State{$\mathtt{push}(v, H)$}
%\If{$|H| > k$}
%\State{$\mathtt{pop}(H)$}
%\EndIf
%\EndIf
%\EndFor
%\EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

\begin{algorithm}[ht]
\caption{Proposed algorithm (query)}
\begin{algorithmic}[1]
\Procedure{Query}{$u$}
\State{Enumerate $S := \{ v | \delta_H(u_\mathrm{left}) \cap \delta_H(v_\mathrm{left}) \neq \emptyset \}$}
\State{Prune $S$ by L1 and L2 bound}
\For{$v \in S$}
 \State{Perform Algorithm~\ref{alg:singlepair} $R=10$ times to roughly estimate $s(u,v)$.}
   \If{The estimated score $s(u,v)$ is not small}
     \State{Perform Algorithm~\ref{alg:singlepair} $R=100$ times to  estimate $s(u,v)$ more accurately}
 \EndIf
\EndFor
\State{Output top $k$ similar vertices}
\EndProcedure
\end{algorithmic}
\end{algorithm}



==> sigmod/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we consider the similarity search problem
that finds top-$k$ similar vertices from a given vertex $u$,
and propose a very efficient and scalable algorithm.

Our algorithm is based on the new formulation of SimRank, called linear recurrence formulation.
Due to this linear recursive formula, single-pair SimRank score $s(u,v)$ can be computed very efficiently by Monte-Carlo simulation (indeed the time complexity is independent of size of graphs).
We also observe that SimRank score $s(u,v)$ decays very rapidly as distance of the pair $u, v$ increases.
By this observation, we establish upper bounds of SimRank score $s(u,v)$ that only depend on  distance $d(u,v)$. The upper bounds can be efficiently computed by Monte-Carlo simulation (in our preprocess). Moreover these upper bounds, together with some adaptive sample technique, allow us to effectively prune the similarity search procedure.
%Combining these ingredients, we proposed a very efficient and scalable similarity search algorithm to find top-$k$ similar vertices from a given vertex $u$, which is based on SimRank scores.

Our experiments show that the proposed algorithm
can compute top-20 similar vertices
in less than a few seconds for graphs of billions edges and in less than a second for graphs of one hundred millions edges, respectively.
%Some state-of-the-art algorithm (i.e., Fogaras and Racz~\cite{FR05}  Monte-Carlo type algorithm) may be faster than ours in query time, but it does not scale up
%to large graphs, due to the space constraint.
Our algorithm requires smaller memory space than any other existing algorithms, which allows our algorithm to scale for much larger graphs
(i.e., graphs with at least a billion edge for the first time).


==> sigmod/contribution.tex <==
\section{Contributions}

\subsection{Problem setting}

%Let us first observe that
%the following is the three fundamental problems for SimRank: We are given a graph $G=(V,E)$.
%\begin{itemize}
%\item \emph{Single-pair SimRank}: Given two vertices $u, v \in V$. Compute the SimRank score $s(i,j)$.
%\item \emph{Single-source SimRank}: Given a vertex $u \in V$. Compute the SimRank score $s(i,j)$ for all $j \in V$.
%\item \emph{All-pairs SimRank}: Compute the SimRank score $s(u,v)$ for all $u, v \in V$.
%\end{itemize}

\drop{
In this paper, we consider the similarity search problem for SimRank (see the formula \eqref{eq:DefinitionOfSimRankEntrywise} for the definition of SimRank).
Usually, there are three fundamental problems for SimRank:
(1) single-pair SimRank to compute $s(u,v)$ for given two vertices $u$ and $v$,
(2) single-source SimRank to compute $s(u,v)$ for a given vertex $u$ and all other vertices $v$,
and (3) all-paris SimRank to compute $s(u,v)$ for all pair of vertices $u$ and $v$.
}

In this paper, we consider a somewhat different problem, called ``The top-$k$ similarity search problem'', as follows:
\begin{problem}[Top-$k$ similarity search]\ \label{prob:problem1}
\begin{itemize}
\item {\rm Given: A graph $G = (V,E)$.}
\item {\rm Query: A query vertex $u$ and a positive integer $k$.}
\item {\rm Output: Top-$k$ vertices with the $k$ highest SimRank similarities with respect to a query vertex $u$.}
\end{itemize}
\end{problem}
%We are also interested in computing the top $k$ similar vertices for all vertices:
%\begin{problem}[Top-$k$ similarity search for all]\ \label{prob:problem}
%\begin{itemize}
%\item {\rm Given: A graph $G=(V,E)$ and a positive integer $k$.}
%\item {\rm Output: Top-$k$ vertices with the $k$ highest SimRank similarities
%for each vertex $u \in V$.}
%\end{itemize}
%\end{problem}
This problem is a special case of the single-source SimRank problem,
since our problem only needs $k$ highly-similar vertices.
%These problems are designed not to compute exact SimRank scores of top-$k$ vertices but to rank top-$k$ vertices
%with respect to SimRank scores of these $k$ vertices.
There are two advantages and reasons for this.

Firstly, this problem could be possibly solved more efficiently.
%than
%the fundamental three problems for SimRank.
More precisely, as pointed above, the difficulty of
computing SimRank score $s(u,v)$ for two vertices $u,v$ comes from
\eqref{eq:DefinitionOfSimRankEntrywise} which is defined recursively.
Thus we have to compute SimRank scores for all pairs of vertices, and hence it requires $O(n^2)$ space.
On the other hand, the top-$k$ similarity search problem has only $k$ outputs for each vertex.
%and only $nk$ outputs even for all vertices.
%Hence the main challenge would be to obtain a sublinear algorithm
%for problem~\ref{prob:problem1}.
Furthermore,
since we do not have to compute the exact SimRank scores,
we are allowed to use some ``approximation'' techniques.
This could also help accelerating algorithms.

Secondly, in practice, there are usually only small number of vertices (e.g., 10 to 20 vertices)
that have high SimRank scores for a query vertex $u$ (e.g., greater than $10^{-2}$).
Since in many applications we are only interested in ``very'' similar vertices,
%we definitely need to find only small number of vertices that have high
%In many applications, we do not interest in ``non-similar'' vertices
%We shall empirically verify this fact in Section \ref{sec:correctness}.
%Under this circumference, we definitely need to find only small number of vertices that have high
%SimRank scores, and hence
it makes sense to consider only ''top-$k$'' vertices for a query vertex $u$, rather
than to compute SimRank scores $s(u,v)$ for all vertices $v \in V$.
%(see the problem ``Top-$k$ similarity search for a single vertex'')
%
%Furthermore, the most of users of real applications do not interested the similarity score itself.
%many real applications attains much importance
%for the similarity ranks, and not the scores.
%For example, many web search engines use both link structure and textual information
%to return the ``related pages'' queries.
%
%
%web pages is motivated by the ``related pages'' queries of web search engines and web document classification.
%Therefore, we can extract similarities from both the textual content of pages and the hyperlink structure.
%In order to combine hyperlink information with information from documents,
%we rather need to figure out ranking of ``top-$k$ vertices'', based on SimRank scores.

\drop{
Thirdly, from a practical view, ranking of top-$k$ nodes is more valuable than knowing
scores of top-$k$ nodes for many real applications~\cite{langville2006google}.
%exact SimRank scores of top-$k$ vertices may be too much.
Specifically, the development of similarity search algorithms between
web pages is motivated by the ``related pages'' queries of web search engines and web document classification.
%Therefore, we can extract similarities from both the textual content of pages and the %hyperlink structure.
In order to combine hyperlink information with information from documents,
we rather need to figure out ranking of ``top-$k$ vertices'', based on SimRank scores.
}

\subsection{Our main contributions and overview}

We propose a novel method that can efficiently
find top-$k$ similar vertices, based on SimRank.
Our algorithm is scalable to graphs of billions edges.
%(i.e., both Problems \ref{prob:problem1} and \ref{prob:problem}).
%This can be achieved by (1) formulating SimRank computation in a noniterative similarity way and (2) Monte Carlo based approach.
%

Technically,
our algorithm is based on the following four key ingredients:
\begin{enumerate}
\item We first establish a new framework of computing SimRank, which introduces a ``linear'' recursive formula for SimRank.
\item Based on this linear recursive formula, single-pair SimRank score $s(u,v)$ can be computed very efficiently by Monte-Carlo simulation. Indeed, the time complexity is independent of the size of networks (e.g., $n, m$).
\item We observe that SimRank score $s(u,v)$ decays very rapidly as distance of the pair $u, v$ increases.
\item By the above observation, we establish upper bounds of SimRank score $s(u,v)$ that only depend on  distance $d(u,v)$. The upper bounds can be efficiently computed by Monte-Carlo simulation (in our preprocess).

    These upper bounds, together with some adaptive sample technique,  allow us to effectively prune the similarity search procedure.
\end{enumerate}
%In addition, our algorithm gives almost exact top-$k$ vertices, see %Subsection~\ref{error}.
Combining these ingredients,
we can obtain the following algorithm for top-$k$ similarity search problem (Problem~\ref{prob:problem1}).

There are two phases: (1) the preprocess phase (for the fourth ingredients) and
(2) the query phase with respect to a query vertex $u$ (to obtain top-$k$ vertices for $u$).
%

We first perform preprocess to compute the auxiliary values
for upper bounds of SimRank $s(u,v)$ for all $v \in V$ (see Section~\ref{sec:upperbound}).
In addition, we construct an auxiliary bipartite graph $H$ as in Section 7.1. This graph $H$ allows us to enumerate ``candidates'' of highly similar vertices $v$ more accurate.
%Finally, we use the adaptive sample technique.
%Specifically, for a query vertex $u$,
%we first compute SimRank scores for each candidate $v$
%to roughly estimate SimRank scores (i.e, we only perform small number
%of random walks for $v$), and throw away some candidates that
%could have small SimRank scores.
%Then, we re-compute more accurate SimRank scores
%for each candidate $v$ that has high estimated SimRank scores
%(i.e., we perform more random walks for $v$).
This is our preprocess phase. The time complexity is $O(n)$.

We now perform our query phase.
We compute SimRank scores $s(u,v)$ for each vertex $u$ in the ascending order of distance from a given vertex $u$, and at the same time, we perform ``pruning'' by the upper bounds obtained in the fourth ingredient.
Each $s(u,v)$ computation is very efficient by the second ingredient.
By the third ingredient,
all top-$k$ vertices (with respect to $u$) are close to $u$ (in the sense of graph distance).
In addition, we use the adaptive sample technique.
Specifically, for a query vertex $u$,
we first estimate SimRank scores roughly for each candidate $v$
(i.e, we only perform small number
of random walks for $v$).
Then, we re-compute more accurate SimRank scores
for each candidate $v$ that has high estimated SimRank scores
(i.e., we perform more random walks for $v$. For more details, please see Section 7.2).

In summary, our search procedure finds all top-$k$ vertices
efficiently by checking the upper bounds and performing the adaptive sampling, and moreover it terminates very quickly (since it only looks
at local area, i.e, vertices that are close to $u$).
%This allows us to find all top-$k$ vertices
%without looking at the whole network.
The time complexity is $O(n)$ in the worst case, but our experiments in Section \ref{sec:experiment}
shows that it is indeed much faster, see below. %sublinear (or even $O(1)$ for most of query vertices in $G$).


We can actually perform the similarity search for all vertices.
We simply apply the above similarity search procedure for each vertex $u$.
The time complexity is $O(n^2)$ in the worst case but it is much faster in practice. The space complexity is $O(m+kn)$, where $kn$ comes from the number of outputs.
%if we want to store all top-$k$ vertices, it only requires $O(k n)$ space.
It is also worth noting that our algorithm is distributed computing friendly.
The bottleneck of the algorithm is computing single-source SimRank scores locally, as described above,
but this part can be performed independently.
Therefore if there are $M$ machines, the running time of our algorithm is $O(n^2/M)$, i.e., reduced by a factor $M$\footnote{indeed, it would be much faster, since in practice
our proposed algorithm for Problem 1 would be much faster}.

%If we have $M$ machines,
%we assign initial vertices to each computer and compute the single-source SimRank independently.
%Thus the computational time is $o(n^2/M)$ or $O(kn / M)$.

In summary, our algorithm has the following attractive characteristics:
\begin{enumerate}
\item
{\bf Small space:} It requires $O(n)$ space for storing the preprocess results.
In addition, for both the single-source case and all vertices case, the algorithm uses only $O(m)$ space to store a network.
%
By comparison, almost all previously known algorithms need $O(n^2)$ space.
\item
{\bf Very fast:} For the preprocess phase, the time complexity is $O(n)$ (see Section~\ref{sec:algorithm}).

Concerning the query phase: for the single-source case (Problem 1),
the time complexity is $O(n)$ in the worst case but much faster in practice.
For all vertices case, the time complexity is $O(n^2)$ in the worst case but much faster in practice.
%By comparison, the solution based on the iterative approach in the original paper %\cite{JW02} requires
%$O(T n^2 d^2)$ time.
\item

{\bf Accurate:} Our algorithm computes only ``approximate SimRank''.
However, we empirically show that our algorithm gives almost exact top-$k$ vertices. See Section 8.2 (and Figure 1 in Section 3.3).
\end{enumerate}
Let us observe that for the space complexity, $O(m)$ is optimal, because we have to read all edges of an input graph.

%

We conducted our experiments to implement our proposed algorithm.
Our experiments show that the proposed algorithm
can scale up to billion-size real networks for the single-source case.
Furthermore, since our all-pairs algorithm can easily be parallelized to multiple machines, if there are 100 machines, even for graphs of
billions size, our all-pairs algorithm can output all top-20 vertices in less than 5 days.
To the best of our knowledge, this is the first time to scale up to such large networks. %In fact, scalability of our algorithm is nearly 70 times larger than any other
%existing algorithms.
%This is due to the memory constraint. Our algorithm
%requires much less memory space than any other existing algorithms.

\medskip
\noindent \textbf{Comparison with other existing algorithms.} \quad
We compare our algorithm with the existing ones in Subsection~\ref{sec:Comparison}.
%As a result,
%In comparison to previous studies,
Our algorithms have the following advantages:
\begin{enumerate}
\item
The state-of-the-art all-pairs algorithm, proposed by Yu et al.~\cite{YZLZL12}, requires much more memory, and hence works only for graphs with
at most a million edges.
On the other hand,
our all-pairs algorithm requires much less memory,
therefore it works for a very large networks.
%than the existing all-pairs algorithms, such as Yu et al.~\cite{YZLZL12},
%and hence our algorithm works for a larger networks than their algorithm.
%(Note that the existing algorithm only worked for $n < 1,000,000$ networks).
\item
The state-of-the-art Monte Carlo based single-pair and single-source algorithm by Fogaras and Racz~\cite{FR05} requires much more space than our
algorithm(even for the case $R'=$ 100 samples for their algorithms).
Even though their algorithm can be faster both in preprocess and in query time, their algorithm scales up to
graphs with at most $70,000,000$ edges. In addition, the accuracy of
their algorithm is less than that of our algorithm, see Section 8.2.
%In comparison,
%our algorithm uses much less space than their algorithm, and hence it works
%up to graphs with at least a billion vertices.
\end{enumerate}
The above two comparisons explain why our algorithm is the first to scale up to graphs
of billions edges. Namely, some state-of-the-art algorithm (i.e., Fogaras and Racz~\cite{FR05}  Monte-Carlo type algorithm) may be faster than ours in query time, but it does not scale up
to large graphs, due to the space constraint.
By comparison, our algorithm requires much less memory space than any other existing algorithms, which allows our algorithm to scale for much larger graphs.


%While SimRank has been used in many applications,
%the original approach requires high computational cost. By
%providing solutions in a highly efficient manner, our algorithm would
%allow many more SimRank-based applications to be developed
%in the future.

\subsection*{Organization of the paper}

This paper is organized as follows. %In Section~\ref{sec:related}, we mention several related work.
In Section~\ref{sec:simrank}, we first introduce a ``linear'' recursive formula for SimRank.
Based on this linear recursive formula, single-pair SimRank score $s(u,v)$ can be computed very efficiently by Monte-Carlo simulation. This will be presented in Section~\ref{sec:montecarlo}. SimRank score $s(u,v)$ decays very rapidly as distance of the pair $u, v$ increases. This is shown in Section~\ref{sec:correctness}.
In Section~\ref{sec:upperbound}, the upper bound of SimRank score $s(u,v)$ will be given via our theoretical analysis. Indeed, we give two such upper bounds, one is more effective for a low degree query vertex, and the other is more effective for a high degree vertex. We also present efficiently Monte-Carlo based algorithms to obtain such
two upper bounds in Section~\ref{sec:upperbound}. Note that this is done in our preprocess phase.
In Section~\ref{sec:algorithm} we propose an algorithm for the similarity search problem by combining the above ingredients.
Finally, in Section~\ref{sec:experiment}, we present many experiments to justify our proposed algorithm, and compare with other state-of-the-arts algorithms.
We conclude our paper in Section~\ref{sec:conclusion}.


==> sigmod/correctness.tex <==
%\newpage
\section{Distance correlation of SimRank}
\label{sec:correctness}

Our top $k$ similarity search algorithm performs
single-pair SimRank computations
for a given source vertex $u$ and for other vertices $v$, but we save the time complexity
by pruning. In order to perform this pruning, we need some upper bounds.
This section and the next section are devoted to establish the upper bounds.
%

The important observation of SimRank is
\begin{quote}
SimRank score $s(u,v)$ decays very fast as the pair $u, v$ goes away.
\end{quote}
In this section, we empirically verify this fact in some real networks,
and in the next section, we develop the upper bounds that only depend on distance.
%In this section, we empirically show that SimRank score $s(u,v)$ decays very rapidly as distance of the pair $u, v$ increases.

Let us look at Figure~\ref{fig1}. We randomly chose 100 vertices $u$ and
enumerate top-1000 similar vertices with respect to to a query vertex $u$ (note that these top-1000 vertices are
``exact'', not `approximate'').
Each point denotes the average distance of the $k$-th similar vertex.
To convince the reader,
we also give the average distance between two vertices
for each network by the blue line.

Figure~\ref{fig1} clearly shows much intuitive information.
If we only need to compute top-10 vertices, all of them are within distance two, three, or four.
In real applications, it is unlikely that
we need to compute top-1000 vertices, but even for this case, most of them are within distance four or five.
We emphasize that these distances are smaller than the average distance of two vertices in each network.
%and hence the ``candidates'' of highly similar vertices
%are screened by the distances.
Thus we can conclude that
the ``candidates'' of highly similar vertices
are screened by distances very well.

%Thus we can conclude that
%for real applications of similarity search (with respect to a query vertex $u$),
%almost all high SimRank score vertices have small distance from $u$.
%
%Hence we only need to look at ``local'' information (i.e, we only need to look at induced subgraphs of distance at most three or four from $u$, and we do not need ``global'' computation, because the average distance
%between two vertices in given networks is bigger than the distance we have to consider to compute SimRank.).

\begin{figure}[ht]
  \centering
  \begin{minipage}[b]{.49\linewidth}
    \includegraphics[width=4cm,bb=50 50 410 302]{figures/wiki-Vote.eps}
    \subcaption{wiki-Vote}
  \end{minipage}
  \begin{minipage}[b]{.49\linewidth}
    \includegraphics[width=4cm,bb=50 50 410 302]{figures/soc-Slashdot0902.eps}
    \subcaption{soc-Slashdot0902}
  \end{minipage}

  \begin{minipage}[b]{.49\linewidth}
    \includegraphics[width=4cm,bb=50 50 410 302]{figures/web-BerkStan.eps}
    \subcaption{web-BerkStan}
  \end{minipage}
  \begin{minipage}[b]{.49\linewidth}
    \includegraphics[width=4cm,bb=50 50 410 302]{figures/soc-LiveJournal1.eps}
    \subcaption{soc-LiveJournal1}
  \end{minipage}
  \caption{Distance correlation of similarity ranking. The red points are for distance of top-1000 similar vertices and the blue line is for average distance of two vertices in each network}
  \label{fig1}
\end{figure}

There is one remark we would like to make from Figure~\ref{fig1}. The top-10 highest SimRank vertices in Web graphs
are much closer to a query vertex than social networks. Thus we can also claim that our algorithm would work better for Web graphs than for social networks, because we only look at subgraphs induced by vertices of distance within three (or even two) from a query vertex.
This claim is verified in Section~\ref{sec:experiment}.


==> sigmod/introduction_sigmod.tex <==
\section{Introduction}
\label{sec:introduction}

\subsection{SimRank}

Recent advances in social and information science have shown that linked data pervades our society.
Since graphs are an intuitive abstraction that can naturally capture objects as well as their relationships as links,
they are becoming increasingly important to represent complicated structures and schema-less data.
%
Much effort has been devoted to extracting useful information from large graphs, % in research community.
and many applications
(e.g., link prediction~\cite{LK07}, graph clustering~\cite{YHY06,ZCY09},
spam detection~\cite{GGP04,ben06}, collaborative tagging analysis~\cite{JCLHD09}, and recommender systems~\cite{AM07})
show some success of vertex similarities and similarity search methods.

The development of similarity measures and similarity search algorithms is motivated by the
applications for web search engines and web document classifications.
%``related pages'' queries of web search engines and web document classification.
Both applications require efficient evaluation of an underlying similarity function,
which extracts proximity from either the textual content of pages and/or the hyperlink structure.
In recent years, contextual data of web pages become drastically complicated.
In addition, link structure is much more homogeneous and language independent source of information.
Furthermore, it is more resistant against spamming.
So many researchers have focused on link-based similarity measures, which only use hyperlink information.
Several link-based similarity functions have been suggested over the web graph.
For example, bibliographic coupling~\cite{Kes63}, co-citation~\cite{Sma73},
SimRank~\cite{JW02}, P-Rank~\cite{ZHS09},
PageSim~\cite{LKL06}, Extended Nearest Neighborhood Structure~\cite{LLK07}, MatchSim~\cite{LLK12}, and so on.

\subsection{SimRank}

Several similarity measures have been proposed.
For example, bibliographic coupling~\cite{Kes63}, co-citation~\cite{Sma73}, P-Rank~\cite{ZHS09},
PageSim~\cite{LKL06}, Extended Nearest Neighborhood Structure~\cite{LLK07}, MatchSim~\cite{LLK12}, and so on.
In this paper, we consider \emph{SimRank} that was introduced by Jeh and Widom~\cite{JW02}.
They observed that ``two similar pages are linked from many similar pages.''
Due to this observation, SimRank is defined as the following, recursively.
\begin{align}
\label{eq:DefinitionOfSimRankEntrywise}
s(u,v) = \begin{cases}
1 & (u = v), \\
\displaystyle \frac{c}{|\delta(u)| |\delta(v)|} \sum_{\substack{u' \in \delta(u), v' \in \delta(v)}} s(u',v') & (u \neq v),
\end{cases}
\end{align}
where $\delta(u)$ denotes in-links of a vertex $u$ and
$c \in (0,1) $ denotes a locality parameter, called a \emph{decay factor},
which is usually set to $c = 0.8$~\cite{JW02} or $c = 0.6$~\cite{LVGT08}.
%
%In many applications, such as natural language processing~\cite{C10}, % Lexicon Induction
%computational advertisement~\cite{AMC08}, % query rewriting
%collaborative filtering~\cite{YSY10},
%web analysis~\cite{JW02}, and so on,
SimRank and related similarity measures give high-quality results
than other similarity measures, such as bibliographic coupling or co-citation.
The reason is that SimRank exploits information on ``multi-step neighborhoods''
while other similarity measures, such as bibliographic coupling or co-citation, utilize only the one-step neighborhoods of pages.
%
%the information in ``multi-step neighborhoods'' while other similarity measures, such as bibliographic coupling or co-citation, utilize only the one-step neighborhoods of pages.
%This is a similar reason for PageRank, as used by the Google search engine, because both SimRank and PageRank can
%take ``global'' information of given networks into account.
%
%%% (comment: PageRank is the ``importance score'' hence it is natural to use the global score.
%%%           Hence ``similar reason'' is, perhaps, incorrect)

%The difficulty of computing SimRank may be viewed as follows: as in \cite{YZLZL12},
%SimRank score $s(.,.)$ can be seen as a random walker defined on a vertex-pair graph $G^2$ that has exactly $n^2$ vertices.
%This means that we may have to apply a matrix-based approach to this graph of order $n^2$, and hence
%the computation cost (both in time and in space) may be expensive (we need at least $n^2$ for both time complexity and space complexity).
%% (comment: the above is incorrect.)

%In order to to reduce the computation cost of SimRank, several
%approximate approaches have been proposed, e.g.,
%\cite{FR05,HFLC10,LHHJSYW10,LLYHD10,LVGT08,YLL10,YLZCP13,YZLZL12}).
%However, these approaches use either spectral decomposition or iterative
%computation. Both the spectral based algorithms and the iterative algorithms retain the
%global characteristic; similarities of all vertex pairs must be
%computed even though only a portion of them are required
%in similarity search.


\subsection{SimRank computation}

Although SimRank gives high-quality similarity measure,
it is not so widely used in practice, due to high computational cost.
While there are several algorithms proposed so far to compute SimRank scores,
unfortunately, their computation complexities (in both time and space) are very expensive.
%
The difficulty of computing SimRank may be viewed as follows:
to compute a SimRank score $s(u,v)$ for two vertices $u,v$,
since \eqref{eq:DefinitionOfSimRankEntrywise} is defined recursively,
we have to compute SimRank scores for all pairs of vertices.
Therefore, since the number of pairs is $O(n^2)$,
it requires $O(n^2)$ space and $O(n^2)$ time, where $n$ is always the number of vertices in $G$\footnote{$m$ is always the number of edges in $G$}.

In order to reduce this computation cost, several approaches have been proposed~\cite{FR05,HFLC10,LHHJSYW10,LLYHD10,LVGT08,YLL10,YLZCP13,YZLZL12}.
Here, we briefly survey some existing computational techniques for SimRank.
We summarize the existing results in Table~\ref{tbl:Complexity}.
Let us point out that there are three fundamental problems for SimRank:
(1) single-pair SimRank to compute $s(u,v)$ for given two vertices $u$ and $v$,
(2) single-source SimRank to compute $s(u,v)$ for a given vertex $u$ and all other vertices $v$,
and (3) all-pairs SimRank to compute $s(u,v)$ for all pair of vertices $u$ and $v$.
%However, these approaches use either spectral decomposition or iterative
%computation. Both the spectral based algorithms and the iterative algorithms retain the
%global characteristic; similarities of all vertex pairs must be
%computed even though only a portion of them are required
%in similarity search.

In the original paper by Jeh and Widom~\cite{JW02},
all-pairs SimRank scores are computed by recursively evaluating the
equation \eqref{eq:DefinitionOfSimRankEntrywise} for all $u, v \in V$.
This ``naive'' computation yields an $O(T d^2 n^2)$ time algorithm, where $T$ denotes the number of iterations
and $d$ denotes the average degree of a given network.
Lizorkin et al.~\cite{LVGT08} proposed a ``partial sum'' technique,
which memorizes partial calculations of Jeh and Widom's algorithm
to reduce the time complexity of their algorithm.
This leads to an $O(T \min \{n m, n^3 / \log n \} )$ algorithm.
Yu et al.~\cite{YZLZL12} applied the fast matrix multiplication~\cite{S69,W12}
and then obtained an $O(T \min \{n m, n^\omega \} )$ algorithm to compute
all pairs SimRank scores, where $\omega < 2.373$ is the exponent of matrix multiplication.
Note that the space complexity of these algorithms is $O(n^2)$,
since they have to maintain all SimRank scores for each pair of vertices
to evaluate the equation \eqref{eq:DefinitionOfSimRankEntrywise}.
This results is, so far, the state-of-the-art algorithm to compute
SimRank scores for all pairs of vertices.
%Many authors used the truncation technique
%that discards small SimRank scores to reduce the space complexity.
\drop{
Some acceleration techniques are proposed very recently.
Jia et al.~\cite{JLZHD10} removed ``dangling vertices'' of a given network
that have no in-links, and this resulted in
a bit faster algorithm, since SimRank scores of dangling vertices are zero.
Cai et al.~\cite{CCJLHLD09} proposed an algorithm to set some certain threshold to
discard SimRank scores that are smaller than the threshold.
This technique works well for scale-free networks.
Jia et al.~\cite{JCLHD09} proposed an algorithm to maintain only vertex pairs of small distance.
This technique works well for small-world networks.
Although the computation cost of these methods is smaller than that by the original paper by Jeh and Widom~\cite{JW02}, unfortunately, they do not scale to graphs of million sizes.
}

There are some random-walk based algorithms.
Jeh and Widom~\cite{JW02} proposed a random-walk
interpretation of SimRank, which is called a ``random surfer-pair model''.
Let us consider two random walks that start from vertices $u$ and $v$, respectively,
and follow the in-links. Let $u^{(t)}$ and $v^{(t)}$ be the $t$-th position of each random walk, respectively.
The first meeting time $\tau_{u,v}$ is defined by
\begin{align} \label{eq:firstmeetingtime}
  \tau_{u v} = \min_{t} \{ u^{(t)} = v^{(t)} \}.
\end{align}
Then SimRank score is obtained by
\begin{align} \label{eq:randomsurferpair}
s(u,v) = \E[ c^{\tau_{u,v}} ].
\end{align}
%Li et al.~\cite{LLYHD10} use this random surfer-pair model but
%their algorithm to compute all pairs SimRank scores is deterministic, which is an %iterative algorithm to compute the first meeting time.
Fogaras and R\'acz~\cite{FR05} evaluate the right-hand side by
Monte-Carlo simulation with a fingerprint tree data structure, and
they obtained a faster algorithm to compute single pair SimRank score for
given two vertices $u, v$.
This work is relevant to our proposed algorithm because our algorithm is also based on
Monte-Carlo simulation. Moreover, this is the state-of-the-art
Monte-Carlo based algorithm for the single-pair and the single-source SimRank problems.

Some papers proposed spectral decomposition based algorithms
(e.g., \cite{FNSO13,HFLC10,LHHJSYW10,YLL10,YLZCP13}), but there is a mistake
in the formulation of SimRank. On the other hand, their algorithms may output reasonable results.
We shall mention more details about these algorithms in Subsections~\ref{error}.

%Some authors~\cite{LHHJSYW10,FNSO13,YLL10} proposed the spectral decomposition based algorithms.
%Their discussions had a critical mistake in the first step,
%however, their algorithm may output reasonable results (see Subsections~\ref{error}).


To the best of our knowledge,
%all existing algorithms to compute SimRank can scale up to at most $n \le 10,000$ size networks,
%and there is no existing algorithm so far that can
there is no existing algorithm so far that can
compute (single pair) SimRank for $m \ge 20,000,000$ size graphs.
%This is because either the time complexity or the space complexity is
%too expensive.
Indeed in Section~\ref{sec:experiment}, we shall
clarify this fact, due to the space constraint.
issues.

\begin{table*}
\caption{Complexity of SimRank algorithms. $n$ denotes the number of vertices, $m$ denotes the number of edges, $d$ denotes the average degree, $T$ denotes the number of iterations, $R$ is the parameter for the algorithm~\cite{FR05}, and $r$ denotes the rank for low-rank approximation.}
\label{tbl:Complexity}
\centering
{ \small
\begin{tabular}{l|llll}
Algorithm & Type & Time & Space & Technique \\ \hline
%Proposed (Subsection~\ref{sec:computingsimrank}) & Single-pair & $O(T m)$ & $O(m)$ & Linear recursive formulation \\
Proposed (Section~\ref{sec:algorithm}) & Top-$k$ search & $<< O(n)$ & $O(m)$ & Linear recursive formulation \& Monte Carlo \\
Proposed (Section~\ref{sec:algorithm}) & Top-$k$ for all & $<< O(n^2)$ & $O(m)$ & Linear recursive formulation \& Monte Carlo \\
%Proposed & All-pairs (Top-$k$ nodes) & $O(k n)$ & $O(m)$ & \\Monte Carlo Based\\
Li et al.~\cite{LLYHD10} & Single-pair & $O(T d^2 n^2)$ & $O(n^2)$ & Random surfer pair (Iterative) \\
Fogaras and R\'acz~\cite{FR05} & Single-pair & $O(T R)$ & $O(m+n R)$ & Random surfer pair (Monte Carlo)\\
Jeh and Widom~\cite{JW02} & All-pairs & $O(T n^2 d^2)$ & $O(n^2)$ & Naive \\
Lizorkin et al.~\cite{LVGT08} & All-pairs & $O(T \min\{n m, n^3 /\log n\})$ & $O(n^2)$ & Partial sum \\
Yu et al.~\cite{YZLZL12} & All-pairs & $O(T \min\{n m, n^\omega\})$ & $O(n^2)$ & Fast matrix multiplication \\
Li et al.~\cite{LCLHD09} & All-pairs & $O(T n^{4/3})$ & $O(n^{4/3})$ & Block partition \\ %(approximate) \\
Li et al.~\cite{LHHJSYW10} & All-pairs & $O(r^4 n^2)$ & $O(n^2)$ & Singular value decomposition \\
  Fujiwara et al.~\cite{FNSO13} & All-pairs & $O(r^4 n)$ & $O(r^2 n^2)$ & Singular value decomposition \\
Yu et al.~\cite{YLL10} & All-pairs & $O(n^3 + T n^2)$ & $O(n^2)$ & Eigenvalue decomposition\\
\end{tabular}
}
\end{table*}
%\footnotetext{Not mentioned in the paper~\cite{FR05}.}


%Yu et al.~\cite{YLL10} proposed a method that uses the eigenvalue decomposition of transition matrix and
%accelerate the SimRank iteration.
%Li et al.~\cite{LHHJSYW10} proposed the non-iterative SimRank algorithm
%that uses low-rank approximation.
%\cite{FNSO13}
%However, their discussions have critical errors. See Appendix B.
%
% *** He et al.~\cite{HFLC10} has two crucial mistakes so we do not refer this paper.
%   (1) SimRank definition is wrong. ( + (1-c) I ver. ) ... eq. (2)
%   (2) Markov chain argument is completely wrong since W is ``column'' stochastic. ... below eq. (6).
% (2013.09.30, T. Maehara)


==> sigmod/montecarlo.tex <==
%\newpage
\section{Monte Carlo algorithm for \\ single-pair SimRank}
\label{sec:montecarlo}

The computational method based on \eqref{eq:expansionuv} (described in Subsection~\ref{sec:computingsimrank})
is more efficient than any previously proposed algorithm
(indeed this is the first linear time algorithm ($O(Tm)$),
and the first linear space algorithm to compute SimRank score
for a single pair of vertices).

However, since we are interested in much faster computation for the
top-$k$ similarity search problem for a single vertex,
this is not enough, because we consider that the computation time $O(T m)$  is still expensive.
To be more precise, we would like to solve the top-$k$ similarity search problem for all vertices.
In this case, the above algorithm would only yield an $O(Tmn)$ algorithm, which is
definitely too expensive.
%because we would like to solve Problem~\ref{prob:problem} for networks of at least millions size, and
%in order to do this, we need to apply the above algorithm many times to large graphs.

Here we propose a Monte-Carlo algorithm for the Single source SimRank,
which is based on the random-walk interpretation of formula \eqref{eq:expansionuv}.
The algorithm requires only a small number of samples. This algorithm yields
a much faster algorithm for the
top-$k$ similarity search problem for a single vertex.

Let us consider a random walk that starts from $u \in V$ and that follows its in-links,
and let $u^{(t)}$ be a random variable for the $t$-th position of this random walk.
Then we observe that
\begin{align} \label{eq:expectationP}
  P^t e_u = \E[ e_{ u^{(t)}  }].
\end{align}
Therefore, by plugging \eqref{eq:expectationP} to \eqref{eq:expansionuv},
we obtain
\begin{align} \label{eq:expectation}
  s^{(T)}(u,v) = & D_{u v} + c \E[ e_{u^{(1)}} ]^\top D \E[ e_{v^{(1)}} ]  \nonumber \\
                   &+ \cdots + c^{T-1} \E[ e_{u^{(T-1)}} ]^\top D \E[ e_{v^{(T-1)}} ].
\end{align}
Our algorithm computes the expectations in the right hand side of \eqref{eq:expectation}
by Monte-Carlo simulation as follows:
Consider $R$ independent random walks $u^{(t)}_1, \ldots, u^{(t)}_R$ that start from $u \in V$,
and $R$ independent random walks $v^{(t)}_1, \ldots, v^{(t)}_R$ that start from $v \in V$ with $u\not=v$.
Then each $t$-th term of \eqref{eq:expectation} can be estimated as
\begin{align} \label{eq:tthestimate}
  c^t \E[ e_{u^{(t)}} ]^\top D \E[ e_{v^{(t)}} ] \simeq \frac{c^t}{R^2} \sum_{r = 1}^R \sum_{r' = 1}^R D_{u_r^{(t)} v_{r'}^{(t)} }.
\end{align}
We compute the right hand side of \eqref{eq:tthestimate}.
Specifically by maintaining the positions of $u_1^{(t)}, \ldots, u_R^{(t)}$ and $v_1^{(t)}, \ldots, v_R^{(t)}$ by hash tables,
it can be evaluated in $O(R)$ time.
%the right hand side of \eqref{eq:tthestimate} can be evaluated in $O(R)$ time.
Therefore the total time complexity to evaluate \eqref{eq:expectation} is $O(T R)$.
The algorithm is shown in Algorithm~\ref{alg:singlepair}.
We emphasize that this time complexity is independent of the size of networks (i.e, $n, m$)
Hence this algorithm can scale to very large networks.

\begin{algorithm}[ht]
\caption{Monte-Carlo Single-pair SimRank} \label{alg:singlepair}
\begin{algorithmic}[1]
\Procedure{SinglePair}{$u$,$v$}
\State{$u_1 \leftarrow u, \ldots, u_R \leftarrow u$, $v_1 \leftarrow v, \ldots, v_R \leftarrow v$}
\State{$\sigma = 0$}
\For{$t = 0, 1, \ldots, T-1$}
\For{$w \in \{ u_1, \ldots, u_R \} \cap \{ v_1 \ldots, v_R \}$}
\State{$\alpha \leftarrow \#\{ r : u_r = w, r = 1, \ldots, R \}$}
\State{$\beta \leftarrow \#\{ r : v_r = w, r = 1, \ldots, R \}$}
\State{$\sigma \leftarrow \sigma + c^t D_{ww} \alpha \beta / R^2 $}
\EndFor
\For{$r = 1, \ldots, R$}
\State{$u_r \leftarrow \delta_-(u_r)$, $v_r \leftarrow \delta_-(v_r)$, randomly}
\EndFor
\EndFor
\State{\textbf{return} $\sigma$}
\EndProcedure
\end{algorithmic}
\end{algorithm}

We give estimation of the number of samples
to compute \eqref{eq:expectation} accurately, with high probability.
We use the Hoeffding inequality to show the following.

\begin{proposition} \label{prop:bound}
Let $\tilde s^{(T)}(u,v)$ be the output of the algorithm. Then
\begin{align} \label{eq:bound}
  \P \left\{ | \tilde s^{(T)}(u,v) - s^{(T)}(u,v) | \ge \epsilon \right\} \le 4 n T \exp \left( - \epsilon^2 R / 2(1-c)^2 \right).
\end{align}
\end{proposition}
The proof of of Proposition~\ref{prop:bound} will be given in Appendix. By Proposition~\ref{prop:bound},
we have the following.
\begin{corollary}
Algorithm~\ref{alg:singlepair} computes the SimRank score $s^{(T)}(u,v)$ with accuracy $0 < \epsilon < 1$
%in $O(\log(1/\epsilon) \log(2/\delta) / \epsilon^2)$ time,
with probability $0 < \delta < 1$ by setting $R = 2(1-c)^2 \log(4 n T / \delta) / \epsilon^2$.
\end{corollary}



\begin{remark}

Fogaras and Bal{\'a}zs~\cite{FR05} also proposed a Monte-Carlo based single-pair SimRank algorithm
but their algorithm and our algorithm are conceptually different.
Their algorithm is based on the random surfer-pair model of SimRank \eqref{eq:randomsurferpair}.
%proposed by Jeh and Widom~\cite{JW02}:
%\begin{align} \label{eq:randomsurfer}
%  S(u,v) = \E[ c^{\tau_{uv}} ].
%\end{align}
%Here, $\tau_{uv}$ denotes a random variable of the first meeting time of $u$ and $v$, defined by
%\begin{align} \label{eq:firstmeetingtime}
%  \tau_{u v} = \min_{t} \{ u^{(t)} = v^{(t)} \}.
%\end{align}
%where $u^{(t)}$ and $v^{(t)}$ denotes the random walks that start from $u$ and $v$, respectively.
The issue to evaluate \eqref{eq:randomsurferpair} is: how to maintain the random walks,
i.e., it requires some path-maintaining data structure.
Fogaras and Bal{\'a}zs used the fingerprint tree data structure for this purpose.
However, the data structure is much more complicated and hence it becomes a computational bottleneck.

On the other hand, our algorithm is based on \eqref{eq:expectation}.
To evaluate \eqref{eq:expectation}, we only have to store the $t$-th position of
random walks and hence \eqref{eq:expectation} can be computed very efficient.
\end{remark}


==> sigmod/relatedwork.tex <==
\subsection{SimRank}
%\subsection{Related work}
\label{sec:related}
% trick
%\footnotetext{Not mentioned in the paper~\cite{FR05}.}
%\footnotetext{There is a mistake. See Appendix B.}

%We categorized related work into two: Linked-based similarity and similarity computation. Let us look at 
%both points.

%\subsection*{Link-based similarity measures}

%Similarity measures are divided into two classes:
%content-based measures, and link-based measures.
%Content-based measures use content information, such as textual, image, or music information
%and link-based measures use only graph structures.
%In this paper, we are only interested in link-based measures for
%large real networks.
%
%%In this paper, we are only interested in the link-based measures.
%There are many link-based similarity measures, e.g.,
%bibliographic coupling~\cite{Kes63}, co-citation~\cite{Sma73},
%SimRank~\cite{JW02}, P-Rank~\cite{ZHS09},
%PageSim~\cite{LKL06}, Extended Nearest Neighborhood Structure~\cite{LLK07}, MatchSim~\cite{LLK12}, and so on.

The main object of this paper is concerning \emph{SimRank} that was introduced by Jeh and Widom~\cite{JW02}.
The basic idea of SimRank is:
\begin{quote}
two pages are similar if they are referenced by similar pages.
\end{quote}
They formulate this intuition
by the following recursive definition of SimRank:
\begin{align}
\label{eq:DefinitionOfSimRankEntrywise}
s(i,j) = \begin{cases}
1 & (i = j), \\
\displaystyle \frac{c}{|\delta_-(i)| |\delta_-(v)|} \sum_{\substack{i' \in \delta_-(i), j' \in \delta_-(j)}} s(i',j') & (i \neq j),
\end{cases}
\end{align}
where $c \in (0,1) $ is a decay factor,
which is usually set to $c = 0.8$~\cite{JW02} or $c = 0.6$~\cite{LVGT08}.

SimRank and related similarity measures give high-quality scores
in many areas, such as natural language processing~\cite{C10}, % Lexicon Induction
computational advertisement~\cite{AMC08}, % query rewriting
collaborative filtering~\cite{YSY10},
web analysis~\cite{JW02}, and so on.
The reason is that SimRank exploits the information in multi-step
neighborhoods while other similarity measures, such as bibliographic coupling or co-citation, %, Jaccard coefficient of neighbors,
utilize only
the one-step neighborhoods of pages.
This is a similar reason for PageRank, as used by the Google search engine, because both SimRank and PageRank can
take ``global'' information of given networks into account.
%Indeed, both can be defined as the ``random surfer-pairs
%model''.


\textbf{FIX}
While there are several algorithms proposed so far to compute SimRank score, unfortunately, its computation
complexity (in both time and space) is very expensive. The naive (and original) algorithm, which is proposed by
Jeh and Widom~\cite{JW02}, requires $O(Tn^2d^2)$ time for the all-pairs case, where $d$ is the average degree and $T$ denotes the number of iterations, and
$O(n^2)$ space.

In order to to reduce the computation cost of SimRank, several
approximate approaches have been proposed, e.g.,
\cite{FR05,HFLC10,LHHJSYW10,LLYHD10,LVGT08,YLL10,YLZCP13,YZLZL12}).
However, these approaches use either spectral decomposition or iterative
computation. Both the spectral based algorithms and the iterative algorithms retain the
global characteristic; similarities of all vertex pairs must be
computed even though only a portion of them are required
in similarity search.

The difficulty of computing SimRank may be viewed as follows: as in \cite{YZLZL12}, SimRank socre $s(.,.)$
can be seen as a random walker defined on a vertex-pair graph $G^2$ that has exactly $n^2$ vertices. This means
that we may have to apply a matrix-based approach to this graph of order $n^2$, and hence
the computation cost (both in time and in space) may be expensive (we need at least $n^2$ for both time complexity and space complexity).



\subsection{SimRank computation}

Here, we briefly survey the existing computational techniques for SimRank.
In the original paper by Jeh and Widom~\cite{JW02},
SimRank is computed by recursively evaluating the
equation \eqref{eq:DefinitionOfSimRankEntrywise} for all $i, j \in V$.
This ``naive'' computation yields an $O(T d^2 n^2)$ time algorithm, where $T$ denotes the number of iterations
and $d$ denotes the average degree of a network.
Lizorkin et al.~\cite{LVGT08} proposed a ``partial sum'' technique to reduce the
time complexity of the naive algorithm. This leads to an $O(T \min \{n m, n^3 / \log n \} )$ algorithm.
Yu et al.~\cite{YZLZL12} applied the fast matrix multiplication~\cite{S69,W12}
and then obtained an $O(T \min \{n m, n^\omega \} )$ algorithm,
where $\omega < 2.373$ is the exponent of matrix multiplication.
Note that the space complexity of these algorithms is $O(n^2)$,
since they have to maintain all SimRank scores for each pair of nodes
to evaluate the equation \eqref{eq:DefinitionOfSimRankEntrywise}. 
Some acceleration techniques to compute SimRank are proposed very recently.
Jia et al.~\cite{JLZHD10} removed ``dangling nodes'' of a network that have no in-links, and this resulted in
a bit faster algorithm, since SimRank scores of dangling nodes are zero. 
Cai et al.~\cite{CCJLHLD09} proposed an algorithm to set some certain threshold to
discard SimRank scores that are smaller than the threshold.
This technique works well on scale-free networks.
Jia et al.~\cite{JCLHD09} proposed an algorithm to maintain only node pairs of small distance.
This technique works well on small-world networks.
Although the computation cost of these methods is smaller that that by the original paper by Jeh and Widom~\cite{JW02}, unfortunately, it does not scale to graphs of million sizes. 

Jeh and Widom~\cite{JW02} also showed a random-walk
interpretation of SimRank, which is called a ``random surfer-pair model''.
Consider random walks that start from vertices $i$ and $j$
and follow the in-links, and
let $\tau_{i,j}$ be the random variable that denotes the first meeting time of $i$ and $j$.
Then SimRank score is obtained by
$$ s(i,j) = \E[ c^{\tau_{i,j}} ]. $$
Li et al.~\cite{LLYHD10} use this random surfer-pair model but
their algorithm is deterministic, which is an iterative algorithm for the first meeting time. 
Fogaras and R\'acz~\cite{FR05} evaluate the right-hand side by
Monte-Carlo simulation with a fingerprint tree data structure. 
This work is relevant to our proposed algorithm because our algorithm is also based on 
Monte-Carlo simulation. 

However, to the best of our knowledge,
%despite of the quality of SimRank,
%it is not so widely used in application area since
%computing SimRank is considered very expensive.
all proposed algorithms to compute SimRank can scale up to at most $n \le 10,000$ size networks,
and there is no proposed algorithm so far that can
compute SimRank for at least $n \ge 1,000,000$ size networks.



%Since many real networks has dangling nodes, it improves much.
%If a graph has some special structure,
%we can accelerate the SimRank computation.
%If a network has scale-free property (i.e., degree power-law),



Table \ref{tbl:Complexity} summarizes the previously known results.

\begin{table*}
\caption{Complexity of SimRank algorithms. $n$ denotes the number of vertices, $m$ denotes the number of edges, $d$ denotes the average degree. $T$ denotes the number of iterations. \TODO{FUJIWARA}}
\label{tbl:Complexity}
%\small
\centering
\begin{tabular}{l|llll}
Algorithm & Type & Time & Space & Technique \\ \hline
Proposed & Single-pair (Top-$k$ nodes) & $O(k)$ & $O(k)$ & Monte Carlo Based\\
Proposed & Single-source (Top-$k$ nodes) & $O(k)$ & $O(k)$ & Monte Carlo Based\\
Proposed & All-pairs (Top-$k$ nodes) & $O(k n)$ & $O(m)$ & \\Monte Carlo Based\\
Li et al.~\cite{LLYHD10} & Single-pair & $O(T d^2 n^2)$ & $O(n^2)$ & Random surfer pair (Iterative) \\
Fogaras and R\'acz~\cite{FR05} & Single-pair & --- \footnotemark & --- $^1$ & Random surfer pair (Monte Carlo Based) \\
Fujiwara et al.~\cite{FNSO13} & All-pairs & $O(n r)$ & Low rank approximation \\
Jeh and Widom~\cite{JW02} & All-pairs & $O(T n^2 d^2)$ & $O(n^2)$ & Naive \\
Lizorkin et al.~\cite{LVGT08} & All-pairs & $O(T \min\{n m, n^3 /\log n\})$ & $O(n^2)$ & Partial sum \\
Yu et al.~\cite{YZLZL12} & All-pairs & $O(T \min\{n m, n^\omega\})$ & $O(n^2)$ & Fast matrix multiplication \\
Li et al.~\cite{LCLHD09} & All-pairs & $O(T n^{4/3})$ & $O(n^{4/3})$ & Block partition (approximate) \\
Li et al.~\cite{LHHJSYW10} & All-pairs & $O(k^4 n^2)$ & $O(n^2)$ & Singular value decomposition\footnotemark  \\
Yu et al.~\cite{YLL10} & All-pairs & $O(n^3 + T n^2)$ & $O(n^2)$ & Eigenvalue decomposition\\
\end{tabular}
\end{table*}

\footnotetext{Not mentioned in the paper~\cite{FR05}.}


Some papers proposed spectral decomposition based algorithms
(e.g., \cite{FNSO13,HFLC10,LHHJSYW10,YLL10,YLZCP13}). We shall mention more details about these algorithms in the 
next section. 


%Yu et al.~\cite{YLL10} proposed a method that uses the eigenvalue decomposition of transition matrix and
%accelerate the SimRank iteration.
%Li et al.~\cite{LHHJSYW10} proposed the non-iterative SimRank algorithm
%that uses low-rank approximation.
%\cite{FNSO13}
%However, their discussions have critical errors. See Appendix B.
%
% *** He et al.~\cite{HFLC10} has two crucial mistakes so we do not refer this paper.
%   (1) SimRank definition is wrong. ( + (1-c) I ver. ) ... eq. (2)
%   (2) Markov chain argument is completely wrong since W is ``column'' stochastic. ... below eq. (6).
% (2013.09.30, T. Maehara)


==> sigmod/simrank.tex <==
%\newpage
\section{New Computational Framework \\ of SimRank}
\label{sec:simrank}

In this section, we introduce a new computational framework of SimRank.
Our framework introduces the \emph{linear recursive formulation} of SimRank \eqref{eq:linearizedsimrank}
(see below) to ``decompose'' the computational difficulty of SimRank.
%
The framework immediately leads to an efficient deterministic algorithm for SimRank (see Subsection~\ref{sec:computingsimrank})
and a very efficient randomized algorithm for SimRank (see Section~\ref{sec:montecarlo}).
Furthermore, since the framework is easy to analyze, we can establish some upper bounds for SimRank (see Section~\ref{sec:upperbound}),
which are very useful to prune the similarity search. This pruning results in a much faster algorithm.

%Some papers propose spectral decomposition based algorithms
%(e.g., \cite{FNSO13,HFLC10,LHHJSYW10,YLL10,YLZCP13}), and their model is indeed exactly the same as ours below.
%But admittedly our model (as well as the papers mentioned above) would not compute ``exact'' SimRank scores, but something similar. On the other hand, our empirical study shows that
%this does not very much change SimRank scores, see Section \ref{sec:experiment}. For more details,
%see Subsection \ref{error}.


\subsection{Linear recursive formulation}

We first introduce a matrix notation of SimRank.
Let $P$ be a transition matrix of the transposed graph $G^\top$, i.e.,
\begin{align*}
P_{ij} = \begin{cases}
1 / |\delta_-(j)| & (i,j) \in E, \\
0 & (i,j) \not \in E.
\end{cases}
\end{align*}
Let $S := (s(i,j))_{ij}$ be a matrix whose $(i,j)$ entry is the SimRank score of $i$ and $j$ (such a matrix
$S$ is called a \emph{SimRank matrix}).
Then the SimRank equation~\eqref{eq:DefinitionOfSimRankEntrywise} is simply represented by
\begin{align} \label{eq:SimRank}
  S = (c P^\top S P) \lor I,
\end{align}
where $\lor$ denotes the entry-wise maximum, i.e., $(A \lor B)_{ij} := \max \{ A_{ij}, B_{ij} \}$.

The difficulty of computing SimRank stems from the recursion \eqref{eq:SimRank}.
This is hard to compute because we have to figure out the entry-wise maximum each time (i.e., non-linear recursion)\footnote{This is the exactly the place where the papers (e.g., \cite{FNSO13,HFLC10,LHHJSYW10,YLL10,YLZCP13}) made mistakes. See Subsection \ref{error}}.

In order to overcome this obstacle,
the first main idea of this paper is to establish the \emph{linear recursive formulation} of SimRank, which consists of only linear operations as follows.
Let us introduce the diagonal matrix $D$ such that
\begin{align} \label{eq:linearizedsimrank}
  S = c P^\top S P + D.
\end{align}
Such a matrix always exists because we can take $D := S - c P^\top S P$ for
the SimRank matrix defined by \eqref{eq:SimRank}.
%Note that such matrix $D$ uniquely exists (i.e., set $D := S - c P^\top S P$ for a SimRank matrix $S$).
We call this matrix $D$ the \emph{diagonal correction matrix}.
Using the notion of the diagonal correction matrix, we can define SimRank as follows:
\begin{quote}
SimRank matrix is a matrix that satisfies \eqref{eq:linearizedsimrank} with some diagonal matrix $D$
and $S_{ii} = 1$ for all $i \in V$.
\end{quote}
This important point of this formulation is the following proposition, whose proof will be given in Appendix.
\begin{proposition} \label{prop:linearizedsimrank}
If a matrix $S'$ satisfies \eqref{eq:linearizedsimrank} for some diagonal matrix $D$, and $S'_{ii} = 1$ for $i \in V$ then $S'$ is equal to the SimRank matrix $S$. The converse is also true.
\end{proposition}
We can also bound the range of $D$ as follows.
\begin{proposition} \label{prop:dbound}
\begin{align} \label{eq:dbound}
  (1-c) \le D_{ii} \le 1.
\end{align}
\end{proposition}
For the proof of Propositions~\ref{prop:dbound}, see Appendix.

%We here show two examples to illustrate the linear formulation of SimRank \eqref{eq:linearizedsimrank}.
We here show an example to illustrate the linear formulation of SimRank \eqref{eq:linearizedsimrank}.
\begin{example} \label{ex:LinearizedSimRank}
Consider the star graph of order $4$ (i.e., a claw).
The transition matrix (of the transposed graph) is
\[
P = \begin{bmatrix}
  0 & 1 & 1 & 1 \\
  1/3 & 0 & 0 & 0 \\
  1/3 & 0 & 0 & 0 \\
  1/3 & 0 & 0 & 0 \\
\end{bmatrix},
\]
and SimRank for $c = 0.8$ is
\[
S = \begin{bmatrix}
  1 & 0 & 0 & 0 \\
  0 & 1 & 4/5 & 4/5 \\
  0 & 4/5 & 1 & 4/5 \\
  0 & 4/5 & 4/5 & 1 \\
\end{bmatrix}.
\]
Since
\[
S - c P^\top S P = \mathrm{diag}(23/75, 1/5, 1/5, 1/5),
\]
we can take $D = \mathrm{diag}(23/75, 1/5, 1/5, 1/5)$ for \eqref{eq:linearizedsimrank}.
Let us emphasis that $D \neq (1 - c) I$.
\end{example}

%\begin{example} \label{ex:completegraph}
%Consider the complete graph with self-loop at every vertices.
%Let $n$ be the number of vertices and
%let $P$ be the transition matrix of the (transposed) graph.
%Then we have $P e_u = \vec{1}/n$ for every vertices $u$.
%By the symmetry, we can assume $D = \lambda I$ for some $\lambda \in \mathbb{R}$.
%Substitute this to \eqref{eq:expansionuvinfinity} we have
%\[
%  1 = \lambda + c \lambda / n + c^2 \lambda/n + \cdots = \lambda \left( 1 + \frac{c / n}{1 - c} \right).
%\]
%Therefore
%\[
%  \lambda = \frac{1 - c}{1 - c + c/n}.
%\]
%Note that if $n = 1$ then $\lambda = 1 -c$ and if $n \to \infty$ then $\lambda \to 1$.
%This shows that $D$ is close to $(1-c)I$ if $n$ is small, and $D$ is close to $I$ if $n$ is large.
%\end{example}

\subsection{Computing SimRank}
\label{sec:computingsimrank}

Having defined our linear recursive formulation \eqref{eq:linearizedsimrank}, we are ready to mention our way to compute SimRank.

For the equation \eqref{eq:linearizedsimrank}, by substituting the left-hand side to the right-hand side recursively,
we obtain the (converging) series: %that converges with rate $O(c^t)$:
\begin{align}
\label{eq:expansion}
  S = D + c P^\top D P + c^2 P^{\top 2} D P^2 + \cdots.
\end{align}
Therefore the SimRank score $s(u,v)$ is obtained from $(u,v)$ component of \eqref{eq:expansion} by
%See Appendix for convergence proof.
%This series converges (see: Appendix). %with rate $O(c^t)$.
%for each $u$ and $v$,
%\begin{align}
%  s^{(T)} (u,v) &= e_u^\top \left(\sum_{t=0}^{T-1} c^t P^{\top t} D P^t\right) e_v \\
%  & = \sum_{t=0}^{T-1} c^t (P^t e_u) D P^t e_v  \\
%  & \le \sum_{t=0}^{T-1} c^t (\max_{ij} D_{ij}) \le 1/(1-c).
%\end{align}
%is a upper bounded monotone nondecreasing sequence in $T$
%and $s^{(T)}(u,v) \to s(u,v)$ for $T \to \infty$.
%
%Once the diagonal correction matrix $D$ is obtained,
%
%{\bf need to fix}
%
%Let $e_i$ be the $i$'th unit vector ($i = 1, \ldots, n$).
%The SimRank score $S_{ij}$ is obtained by $e_i^\top S e_j$.
%Hence, by applying $e_i^\top$ and $e_j$ to the both-hand sides of
%\eqref{eq:NeumannExpansion}, we obtain
%\begin{align*}
%S_{ij}
%= e_i^\top D e_j + c (P e_i)^\top D P e_j + c^2 (P^2 e_i)^\top D P^2 e_j + \cdots.
%\end{align*}
%
%{\bf Replace}
%
%Let $u, v \in V$. Then
\begin{align} \label{eq:expansionuvinfinity}
  s(u,v) &= e_u^\top S e_v \nonumber \\
  &= e_u^\top D e_v + c (P e_u)^\top D P e_v + c^2 (P^2 e_u)^\top D P^2 e_v + \cdots.
  %\sum_{t = 1}^\infty c^k (P^j e_u)^\top D P^k e_u.
\end{align}
Let $s^{(T)}(u,v)$ be the sum of $T$-th terms of the above equation:
\begin{align} \label{eq:expansionuv}
s^{(T)}(u,v) :=& e_u^\top D e_v + c (P e_u)^\top D P e_v \nonumber \\
             & + \cdots + c^{T-1} (P^{T-1} e_u)^\top D P^{T-1} e_v.
\end{align}
Then $s^{(T)}(u,v)$ converges to $s(u,v)$ with rate $c^T$.
More precisely, it is straightforward to see that
\begin{align} \label{eq:error}
  0 \le s(u,v) - s^{(T)}(u,v) \le \frac{c^T}{1 - c}.
\end{align}
This implies that
if we want to compute $s(u,v)$ with accuracy less than $\epsilon > 0$,
we just need to compute $s^{(T)}(u,v)$ by taking $T = \ceil{ \log(\epsilon (1-c)) / \log c }$.
%take the sum up to $T \ge (\log \epsilon / \log c)$-th term of the above equation:
This yields an algorithm whose time and space complexity is $O(T m)$ and $O(n)$ space, respectively.

As claimed in Section~\ref{sec:introduction}, we would like to make this time complexity faster.
For this purpose,
in the rest of the paper we focus on computing $s^{(T)}(u,v)$, instead of $s(u,v)$.


\subsection{Estimating diagonal correction matrix}
\label{error}

Estimating the diagonal correction matrix $D$ is a hard task.
Indeed it is as difficult as computing the SimRank matrix $S$ itself.
Hence we need an easily computable approximation of $D$.


Recall that some papers use the following SimRank ``definition'', which is indeed incorrect:
\begin{align} \label{eq:wrongsimrank}
  S' = c P^\top S' P + (1 - c) I.
\end{align}
(e.g., equation (2) in \cite{LHHJSYW10}, equation (2) in \cite{HFLC10}, equation (3) in \cite{YLZCP13}, and equation (2) in \cite{FNSO13}).
%However, this is different from the original SimRank.
This recursion does not provide the original SimRank
because $S'$ does not necessary satisfy $S'_{ii} = 1$ ($i = 1, \ldots, n$);
%see Example~\ref{ex:LinearizedSimRank} and \ref{ex:completegraph} for counterexamples.
see Example~\ref{ex:LinearizedSimRank} for a counterexample.

However, if we regard \eqref{eq:wrongsimrank} as an ``approximation'' of $D$, i.e., $D \simeq (1 - c) I$,
the situation is much better for the similarity search problem.
Because, in practice, this approximation does not much affect
top-$k$ similarity rankings (``approximate''
SimRank scores could be different from the ``exact'' SimRank scores, though),
in this paper, we simply approximate $D \simeq (1-c) I$,
as other papers did (e.g., \cite{FNSO13,HFLC10,LHHJSYW10,YLL10,YLZCP13}).
We now give practical justifications for
approximating $D \simeq (1 - c) I$.
%We first evaluate the accuracy of our algorithm in small networks.
%Recall that our algorithms has two ``approximation''
%in diagonal estimation $D \simeq (1-c)I$ and
%Monte-Carlo simulation (approximate expectations by empirical expectations).
Figure~\ref{fig:Dapprox} shows the scatter plot of
exact SimRank scores  and approximated SimRank scores (based on \eqref{eq:linearizedsimrank}) for highly similar vertices.
We can see that the points are in a straight line of slope one (in log-log plot).
This means that
%(1) The similarity ranking is accurately computed.
the approximation $D \simeq (1-c) I$ only changes the scale of each SimRank score
and hence it does not affect the similarity ranking.

Note that our proposed method does not depend on
the approximation $D \simeq (1-c) I$.
Hence if we estimate $D$ more accurately, the result also becomes more precisely.
Therefore, in the rest of the paper
we keep using the symbol ``$D$'' to denote $(1 - c) I$,
to emphasize this point. % and to avoid the confusion.

\begin{remark}
Since our definition \eqref{eq:linearizedsimrank} is linear in $D$,
the top-$k$ similarity ranking does not change under the scaling of $D$.
Therefore if the ``exact'' diagonal correction matrix $D$ is proportional to the identity matrix $I$,
we can exactly finds the top-$k$ similarity ranking by approximating $D \simeq (1-c) I$.
\end{remark}




%We first compute both the exact SimRank scores and the approximate SimRank scores in Figure~\ref{fig:Dapprox}.
%This shows the approximate scores are proportional to the exact scores, i.e., they only differ in scaling.
%More precisely, we compute the ``precision at $k$'', defined by
%\[
%  \textrm{precision at } k = \frac{(\textrm{exact top } k) \cap (\textrm{approximate top } k)}{k},
%\]
%for some dataset networks. The results are shown in Table~\ref{tbl:Dapprox}. This is also performs very well.

\begin{figure}[ht]
  \centering
  \begin{minipage}[b]{.49\linewidth}
    \includegraphics[width=4cm,bb=18 180 594 612]{figures/ca-GrQc.json.approx.0.eps}
    \subcaption{ca-GrQc}
  \end{minipage}
  \begin{minipage}[b]{.49\linewidth}
    \includegraphics[width=4cm,bb=18 180 594 612]{figures/cit-HepTh.json.approx.0.eps}
    \subcaption{cit-HepTh}
  \end{minipage}
  \caption{Correlation of exact SimRank scores and approximated SimRank scores}
  \label{fig:Dapprox}
\end{figure}



==> sigmod/topk.tex <==
%\newpage
\section{Top $k$ SimRank algorithm}
\label{sec:topk}

Our algorithm computes the single-pair SimRank $S(u,v)$ one-by-one, in ascending order of distance.
We maintain the top $k$ similar vertices by min-heap, which can perform $\mathtt{min}$, $\mathtt{insert}$, and $\mathtt{extract\_min}$ operations efficiently.
The algorithm is shown in Algorithm~\ref{alg:topk}.

\begin{algorithm}[ht]
\caption{Top $k$ SimRank} \label{alg:topk}
\begin{algorithmic}[1]
\Procedure{TopK}{$u, k$}
\State{Initialize a min-heap $H$}
\For{$d = 1, 2, \ldots$}
\State{Compute $\gamma(d)$}
\If{$|H| = k$ and $\mathtt{min}(H).\textrm{key} \ge \gamma(d)$}
\State{Report all vertices in $H$}
\State{\textbf{return}}
\EndIf
\For{$w \in V \textrm{ with } d(u, w) = d$}
\State{Compute $S(u, w)$}
\If{$|H| < k$}
\State{$\mathtt{insert}(H, (S(u,w), w))$}
\ElsIf{$\mathtt{min}(H).\textrm{key} \ge S(u,w))$}
\State{$\mathtt{extract\_min}(H)$}
\State{$\mathtt{insert}(H, (S(u,w), w))$}
\EndIf
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Efficient Implementation}

To implement Algorithm~\ref{alg:topk} efficiently, 
we can reuse the result of  Monte-Carlo simulation for $P^t e_u$.
At first, by Algorithm~\ref{alg:beta},
we compute $P^t e_u$ and $\beta(d,t)$ for $t = 1, \ldots, T$.
This takes $O(T R)$ time and $O(T R)$ space.
Next, we compute $\gamma(d)$ for all $d = 1, \ldots, T$ by \eqref{eq:gamma}.
This takes $O(T^3)$ time\footnote{Actually, this can be done in $O(T^2)$ time by the range minimum query data structure. However, since $T$ is very small (e.g., $T = 11$ in our experiments), a naive algorithm with $O(T^3)$ is enough fast.}.
Since we have computed $P^t e_u$, 
the SimRank score $S(u, w)$ can be computed in $O(T R)$ with 
simulating only $P^t e_w$.


==> sigmod/upperbound.tex <==
%\newpage
\section{Tight upper bounds}
\label{sec:upperbound}

In the previous section, we observe that
highly similar vertices with respect to a query vertex are within small distance from $u$.
This observation allows us to propose our efficient algorithm
for the top-$k$ similarity search problem for a single vertex (i.e., Problem \ref{prob:problem1}).
%in the following way: we compute SimRank score $s(u,v)$ in ascending order of distance from $u$.
In order to obtain this algorithm,
%
%to complete the algorithm,
we need to establish the upper bounds of SimRank
that depend only on distance, which will be done in this section.
%These upper bounds are very useful to prune the similarity search. This pruning results in a much faster algorithm.

%Our top $k$ similarity search algorithm performs
%single-pair SimRank computations
%for a given source vertex $u$ and other vertices $v$
%with pruning by some upper bounds.
%This section is devoted to establish the upper bounds.
%
%The important observation of SimRank is
%\begin{quote}
%SimRank score $s(u,v)$ decays very fast as the pair $u, v$ goes away.
%\end{quote}
%For example,
%
%
%This fact is verified in Section~\ref{sec:experiment}.

Let us observe that by definition, SimRank score is bounded by
the decay factor to the power of the distance:
\[
  s(u,v) \le c^{d(u,v)}
\]
%However, this bound is too weak.
Since almost all high SimRank score vertices with respect to a query vertex $u$
are located within distance three from $u$ (see Figure~\ref{fig1}),
we obtain $s(u,v) \le c^3 = 0.216$. But this is too large for our purpose (indeed,
our further experiments to compare actual SimRank scores with this bound confirm that it is too large).

Here we propose two upper bounds, called ``L1 bound'' and ``L2 bound''.
Our algorithm, described in a later section, combines these two bounds to perform ``pruning'', which results in
a much faster algorithm.

\subsection{L1 bound}

The first bound is based on the following inequality:
for a vector $x$ and a stochastic vector $y$,
\begin{align} \label{eq:l1}
  x^\top y \le \max_{w \in \mathrm{supp}(y)} x^\top e_w,
\end{align}
where $\mathrm{supp}(y) := \{ w \in V : y(w) > 0 \}$ is a positive support of $y$.
We bound $(P^t e_u)^\top D (P^t e_v)$ by this inequality.

Fix a query vertex $u$.
Let us define
\begin{align} \label{eq:alpha}
  \alpha(u, d, t) := \max_{w \in V, d(u,w) = d} (P^t e_u)^\top D e_w
\end{align}
for $d = 1, \ldots, d_{\mathrm{max}}$ and $t = 1, \ldots, T$,
and
\begin{align} \label{eq:beta}
  \beta(u, d) := \sum_{t=0}^{T-1} c^t \max_{d - t \le d' \le d + t} \alpha(u, d', t)
\end{align}
for $t = 1, \ldots, T$. Here $d_\mathrm{max}$ is distance such that
if $d(u,v) > d_\mathrm{max}$ then $s(u,v)$ is too small to take into account.
(We usually set $d_\mathrm{max} = T$).
\begin{proposition} \label{prop:L1bound}
For a vertex $v$ with $d(u, v) = d$, we have
\begin{align} \label{eq:upperbound1}
  s^{(T)}(u,v) \le \beta(u, d)
\end{align}
\end{proposition}
The proof will be given in Appendix.

\begin{remark}
$\alpha(u, d, t)$ has the following probabilistic representation:
\[
  \alpha(u, d, t) = \max_{d(u,w) = d} D_{ww} \P \{ u^{(t)} = w \}
\]
where $u^{(t)}$ denotes the position of a random walk
that starts from $u$ and follows its in-links.
%If the network has average degree $|\delta|$ then
%this value decreases as $1/|\delta|^{d-t}$
\end{remark}

To compute $\alpha(u,d,t)$ and $\beta(u,d)$,
we can use Monte-Carlo simulation for $P^t e_u$
as shown in Algorithm~\ref{alg:alpha}.

Similar to Proposition~\ref{prop:bound},
we obtain the following proposition, whose proof will be given in Appendix.
This proposition shows that Algorithm~\ref{alg:alpha} can compute $\alpha(u,d,t)$ and $\beta(u,d)$.
\begin{proposition} \label{prop:L1sample}
Let $\tilde \beta(u,d)$ be computed by Algorithm~\ref{alg:alpha}. Then
\begin{align*} %\label{eq:bound}
  \P \left\{ | \tilde \beta(d,t) - \beta(d,t) | \ge \epsilon \right\} \le 2 n d_{\mathrm{max}} T \exp(- 2 \epsilon^2 R)
\end{align*}
\end{proposition}
%The proof of of Proposition~\ref{prop:bound} will be given in Appendix.
By Proposition~\ref{prop:L1sample}, we have the following.
%Proposition~\ref{prop:L1sample} gives the following corollary.
\begin{corollary}
Algorithm~\ref{alg:alpha} computes $\beta(u,d)$ with accuracy less than $0 < \epsilon < 1$
with probability at least $0 < \delta < 1$ by setting $R = \log(2 n d_\mathrm{max} T/\delta) / (2 \epsilon^2)$.
\end{corollary}

\begin{algorithm}[ht]
\caption{Monte-Carlo $\alpha(u,d,t)$, $\beta(u,d)$ computation} \label{alg:alpha}
\begin{algorithmic}[1]
\Procedure{ComputeAlphaBeta}{$u$}
\State{$u_1 \leftarrow u, \ldots, u_R \leftarrow u$}
\For{$t = 0, 1, \ldots, T-1$}
  \For{$w \in \{ u_1, \ldots, u_R \}$}
  \State{$\mu \leftarrow D_{ww} \#\{ r : u_r = w, r \in [1, R]\} / R $}
    \State{$\alpha(u, d(u,w), t) \leftarrow \max \{ \alpha( u, d(u,w), t ), \mu \}$}
  \EndFor
  \For{$r = 1, \ldots, R$}
    \State{$u_r \leftarrow \delta(u_r)$ randomly}
  \EndFor
\EndFor
\For{$d = 1, \ldots, T$}
  \State{$\beta(u,d) = \sum_{t=0}^{T-1} c^t \max_{d - t \le d' \le d + t} \alpha(u, d', t)$}
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{L2 bound}

The second bound is based on the Cauchy--Schwartz inequality:
for nonnegative vectors $x$ and $y$,
\begin{align} \label{eq:l2}
  x^\top y \le \|x\| \|y\|.
\end{align}
We also bound $(P^t e_u) D (P^t e_v)$ by this inequality.

Let
\begin{align} \label{eq:gamma}
  \gamma(u,t) := \| \sqrt{D} P^t e_u \|,
\end{align}
where $\sqrt{D} = \mathrm{diag}(\sqrt{D_{11}}, \ldots, \sqrt{D_{nn}})$.
Note that, since $D$ is a nonnegative diagonal matrix, $\sqrt{D}$ is well-defined.

\begin{proposition} \label{prop:L2bound}
For two vertices $u$ and $v$, we have
\begin{align} \label{eq:upperbound2}
  s^{(T)}(u,v) \le \sum_{t=0}^T c^t \gamma(u,t) \gamma(v,t)
\end{align}
\end{proposition}
The proof of Proposition~\ref{prop:L2bound} will be given in Appendix.

To compute $\gamma(u, d)$ for each $u$,
we can use Monte-Carlo simulation.
Let us emphasize that we can compute $\gamma(u, d)$ for each $u$ and $d \le d_{\mathrm{max}}$ in
preprocess.

The following proposition, whose proof will be given in Appendix, shows that Algorithm~\ref{alg:gamma}
can compute $\gamma(u, d)$.
\begin{proposition} \label{prop:L2sample}
Let $\tilde \gamma(u,t)$ be computed by Algorithm~\ref{alg:gamma}. Then
\begin{align*} %\label{eq:bound}
  \P \left\{ | \tilde \gamma(u,t) - \gamma(u,t) | \ge \epsilon \right\} \le 4 n \exp \left( -\epsilon^2 R / 8 \right).
\end{align*}
\end{proposition}
The proof of of Proposition~\ref{prop:L2sample} will be given in Appendix. By
Proposition~\ref{prop:L2sample}, we have the following.
\begin{corollary}
Algorithm~\ref{alg:gamma} computes $\gamma(u,t)$ with accuracy less than $0 < \epsilon < 1$
with probability at least $0 < \delta < 1$ by setting $R = 8 \log(4 n/\delta) / \epsilon^2$.
\end{corollary}

\begin{algorithm}[ht]
\caption{Monte-Carlo $\gamma(u,t)$ computation} \label{alg:gamma}
\begin{algorithmic}[1]
\Procedure{ComputeGamma}{$u$}
\State{$u_1 \leftarrow u, \ldots, u_R \leftarrow u$}
\For{$t = 0, 1, \ldots, T-1$}
  \State{$\mu = 0$}
  \For{$w \in \{ u_1, \ldots, u_R \}$}
  \State{$\mu \leftarrow \mu + D_{ww} \#\{ r : u_r = w, r \in [1,R] \}^2 / R^2 $}
  \EndFor
  \State{$\gamma(u, t) \leftarrow \sqrt{ \mu }$}
  \For{$r = 1, \ldots, R$}
    \State{$u_r \leftarrow \delta(u_r)$ randomly}
  \EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}


\subsection{Comparison of two bounds}

The reason why we need both L1 and L2 bounds is the following:
The L1 bound is more effective for a low degree query vertex $u$.
This is because if $u$ has low degree then $P^t e_u$ is sparse.
Therefore the bound \eqref{eq:tthbound} becomes tighter.

On the other hand, the L2 bound is more effective for high degree vertex $u$.
This is because if $u$ has high degree then $P^t e_u$ spreads widely,
and hence each entry is small.
Therefore $\| \sqrt{D} P^t e_u \|$ decrease rapidly.
%
%We verify this discussion by real networks in Section 8.
%
%We also use the following heuristical approach.




==> simrank.tex <==
\section{SimRank}



